Fewer Steps, Better Plans: Sampling Variance in Flow-Matching Navigation World Models

Navigation world models use one backbone and one dense multi-step sampler both to generate future frames and to rank candidate plans. We ask whether planning needs the capacity and integration accuracy that generation does. To answer this within one training run, we train MatNWM, whose feed-forward layers nest four granularities, alongside an identically trained monolithic baseline. Using MatNWM as a controlled probe, we find that the two tasks have asymmetric demands. Visual realism requires full granularity and many neural function evaluations (NFEs). In contrast, planning ranks candidates by expected outcome, meaning low-variance cost estimates are required rather than sharp samples. We trace this difference to the optimizer's curse: selecting the best of many noisy single-rollout scores rewards favorable noise. While a single NFE collapses to the conditional mean and distorts sharp turns, we show that averaging two 2-NFE rollouts balances both effects, and coarse Euler integration provides stable cost estimates without retraining. To this end, few-step Euler alone makes 49-NFE planning $11.6\times$ faster with no loss in accuracy. Utilizing MatNWM's smallest granularity further raises this speedup to $15.4\times$, while realistic future predictions can still be generated with MatNWM at full granularity. We plan to release the model weights and source code.

==> tab/gen/supp_axes_body.tex <==
Depth + FFN & \M{1} & 0.44 & 65 & 0/12 & 12/12 & $+1.1$ & 0/12 & 12/12 & $+0.6$ \\
 & \M{4} & 1.00 & 132 & 1/12 & 12/12 & $+0.5$ & 0/12 & 12/12 & $+0.3$ \\
\addlinespace[2pt]
Heads + FFN & \M{1} & 0.27 & 46 & 1/12 & 12/12 & $+2.2$ & 1/12 & 12/12 & $+2.6$ \\
 & \M{4} & 1.00 & 109 & 0/12 & 12/12 & $+0.3$ & 1/12 & 12/12 & $+0.2$ \\
\addlinespace[2pt]
Heads + depth + FFN & \M{1} & 0.20 & 32 & 3/12 & 8/12 & $+4.0$ & 1/12 & 12/12 & $+3.8$ \\
 & \M{4} & 1.00 & 109 & 3/12 & 9/12 & $+0.8$ & 0/12 & 12/12 & $+0.6$ \\
\addlinespace[2pt]
Hidden width + FFN & \M{1} & 0.20 & 32 & 2/12 & 9/12 & $+5.5$ & 4/12 & 9/12 & $+5.5$ \\
 & \M{4} & 1.00 & 108 & 1/12 & 12/12 & $+0.7$ & 3/12 & 12/12 & $+0.1$ \\
\addlinespace[2pt]
Hidden width + depth + FFN & \M{1} & 0.14 & 21 & 3/12 & 8/12 & $+7.7$ & 5/12 & 9/12 & $+7.0$ \\
 & \M{4} & 1.00 & 110 & 3/12 & 10/12 & $+1.1$ & 1/12 & 12/12 & $+1.0$ \\


==> tab/gen/supp_axes_mid_body.tex <==
Depth + FFN & \M{2} & 0.55 & 81 & 0/12 & 12/12 & $+0.6$ & 0/12 & 12/12 & $+0.6$ \\
 & \M{3} & 0.72 & 102 & 0/12 & 11/12 & $+0.4$ & 0/12 & 12/12 & $+0.5$ \\
\addlinespace[2pt]
Heads + FFN & \M{2} & 0.44 & 59 & 0/12 & 12/12 & $+0.7$ & 0/12 & 12/12 & $+0.8$ \\
 & \M{3} & 0.67 & 81 & 0/12 & 12/12 & $+0.3$ & 0/12 & 11/12 & $+0.5$ \\
\addlinespace[2pt]
Heads + depth + FFN & \M{2} & 0.36 & 47 & 2/12 & 8/12 & $+1.8$ & 0/12 & 12/12 & $+1.5$ \\
 & \M{3} & 0.61 & 73 & 2/12 & 9/12 & $+1.1$ & 0/12 & 11/12 & $+1.1$ \\
\addlinespace[2pt]
Hidden width + FFN & \M{2} & 0.35 & 47 & 0/12 & 10/12 & $+2.9$ & 2/12 & 12/12 & $+2.6$ \\
 & \M{3} & 0.59 & 72 & 0/12 & 10/12 & $+1.5$ & 1/12 & 12/12 & $+1.0$ \\
\addlinespace[2pt]
Hidden width + depth + FFN & \M{2} & 0.27 & 37 & 0/12 & 9/12 & $+4.0$ & 2/12 & 9/12 & $+4.0$ \\
 & \M{3} & 0.53 & 65 & 2/12 & 10/12 & $+2.0$ & 1/12 & 12/12 & $+2.2$ \\


==> tab/gen/supp_b0_curse_body.tex <==
\sacson & \at{4}{50} & $100{\times}5$ & 0.0377 & 0.0426 & 0.88 & $+1.18$\sig \ci{$+1.06$, $+1.32$} & 49\,\% & 17\,\% & -- & 0.94 \ci{0.84, 1.04} \\
\sacson & \at{1}{50} & $500{\times}3$ & 0.0337 & 0.0374 & 0.90 & $+1.22$\sig \ci{$+1.16$, $+1.28$} & 49\,\% & 16\,\% & 1.00 (ref.) & 0.96 \ci{0.89, 1.03} \\
\sacson & \at{1}{5} & $500{\times}3{\times}3$ & 0.0268 & 0.0432 & 0.62 & $+0.73$\sig \ci{$+0.70$, $+0.77$} & 33\,\% & 27\,\% & 0.95 \ci{0.94, 0.95} & 0.94 \ci{0.87, 1.01} \\
\sacson & \at{1}{3} & $500{\times}2{\times}3$ & 0.0208 & 0.0469 & 0.44 & $+0.39$\sig \ci{$+0.37$, $+0.42$} & 20\,\% & 40\,\% & 0.86 \ci{0.85, 0.87} & 0.96 \ci{0.88, 1.05} \\
\sacson & \at{1}{2} & $500{\times}4{\times}3$ & 0.0118 & 0.0471 & 0.25 & $+0.08$\sig \ci{$+0.07$, $+0.09$} & 5\,\% & 68\,\% & 0.75 \ci{0.73, 0.76} & 0.90 \ci{0.83, 0.97} \\
\sacson & \M{1} Heun@3 & $100{\times}3$ & 0.0196 & 0.0416 & 0.47 & $+0.49$\sig \ci{$+0.42$, $+0.57$} & 24\,\% & 31\,\% & 0.96 \ci{0.96, 0.97} & -- \\
\sacson & \M{1} Midpoint@3 & $100{\times}3$ & 0.0245 & 0.0417 & 0.59 & $+0.76$\sig \ci{$+0.66$, $+0.87$} & 35\,\% & 22\,\% & 0.98 \ci{0.98, 0.99} & -- \\
\midrule
\recon & \at{1}{50} & $500{\times}3$ & 0.0257 & 0.0381 & 0.67 & $+1.21$\sig \ci{$+1.17$, $+1.26$} & 47\,\% & 13\,\% & 1.00 (ref.) & 1.39 \ci{1.30, 1.48} \\
\recon & \at{1}{5} & $500{\times}3{\times}3$ & 0.0206 & 0.0448 & 0.46 & $+0.69$\sig \ci{$+0.67$, $+0.71$} & 30\,\% & 22\,\% & 0.91 \ci{0.90, 0.91} & 1.39 \ci{1.30, 1.48} \\
\recon & \at{1}{3} & $500{\times}2{\times}3$ & 0.0145 & 0.0482 & 0.30 & $+0.36$\sig \ci{$+0.35$, $+0.38$} & 17\,\% & 33\,\% & 0.79 \ci{0.78, 0.81} & 1.43 \ci{1.33, 1.53} \\
\recon & \at{1}{2} & $500{\times}4{\times}3$ & 0.0046 & 0.0467 & 0.10 & $+0.04$\sig \ci{$+0.04$, $+0.04$} & 2\,\% & 68\,\% & 0.70 \ci{0.69, 0.72} & 1.39 \ci{1.30, 1.49} \\
\recon & \M{1} Heun@3 & $100{\times}3$ & 0.0179 & 0.0404 & 0.44 & $+0.67$\sig \ci{$+0.61$, $+0.73$} & 29\,\% & 24\,\% & 0.94 \ci{0.93, 0.95} & -- \\
\recon & \M{1} Midpoint@3 & $100{\times}3$ & 0.0219 & 0.0415 & 0.53 & $+0.81$\sig \ci{$+0.74$, $+0.88$} & 34\,\% & 20\,\% & 0.99 \ci{0.98, 0.99} & -- \\
\midrule
\scand & \at{1}{5} & $500{\times}3{\times}3$ & 0.0178 & 0.0479 & 0.37 & $+0.40$\sig \ci{$+0.38$, $+0.43$} & 20\,\% & 32\,\% & 1.00 (ref.) & 0.86 \ci{0.82, 0.91} \\
\scand & \at{1}{3} & $500{\times}2{\times}3$ & 0.0133 & 0.0487 & 0.27 & $+0.25$\sig \ci{$+0.23$, $+0.27$} & 14\,\% & 40\,\% & 0.93 \ci{0.93, 0.94} & 0.89 \ci{0.82, 0.96} \\
\scand & \at{1}{2} & $500{\times}4{\times}3$ & 0.0040 & 0.0463 & 0.09 & $+0.03$\sig \ci{$+0.03$, $+0.04$} & 2\,\% & 73\,\% & 0.83 \ci{0.82, 0.84} & 0.91 \ci{0.85, 0.97} \\
\scand & \M{1} Heun@3 & $100{\times}3$ & 0.0140 & 0.0467 & 0.30 & $+0.33$\sig \ci{$+0.28$, $+0.39$} & 18\,\% & 35\,\% & 0.86 \ci{0.85, 0.88} & -- \\
\scand & \M{1} Midpoint@3 & $100{\times}3$ & 0.0174 & 0.0502 & 0.35 & $+0.41$\sig \ci{$+0.36$, $+0.47$} & 21\,\% & 30\,\% & 0.89 \ci{0.87, 0.90} & -- \\


==> tab/gen/supp_b0_oneshot_body.tex <==
\multicolumn{16}{@{}l}{\emph{1-shot direct prediction at 1\,s horizon (zero autoregressive chaining, full test splits: $3{,}416 / 4{,}262 / 1{,}883$ anchors)}} \\
\M{1}, $S{=}50$ (49) & 0.229 & 0.569 & 0.354 & 0.332 & 18.8 & 0.271 & 0.665 & 0.395 & 0.350 & 19.0 & 0.286 & 0.710 & 0.403 & 0.349 & 27.1 \\
\M{1}, $S{=}20$ (19) & 0.220 & 0.540 & 0.350 & 0.329 & 19.0 & 0.262 & 0.635 & 0.391 & 0.348 & 20.0 & 0.276 & 0.678 & 0.399 & 0.346 & 27.2 \\
\M{1}, $S{=}10$ (9) & 0.208 & 0.504 & 0.345 & 0.325 & 19.9 & 0.249 & 0.597 & 0.385 & 0.347 & 21.3 & 0.263 & 0.637 & 0.393 & 0.341 & 27.8 \\
\M{1}, $S{=}5$ (4) & 0.188 & 0.449 & 0.337 & 0.321 & 24.0 & 0.227 & 0.533 & 0.374 & 0.346 & 23.2 & 0.243 & 0.574 & 0.384 & 0.337 & 30.9 \\
\M{1}, $S{=}4$ (3) & 0.178 & 0.424 & 0.335 & 0.322 & 28.1 & 0.216 & 0.502 & 0.369 & 0.347 & 24.4 & 0.232 & 0.544 & 0.380 & 0.336 & 33.9 \\
\M{1}, $S{=}3$ (2) & 0.164 & 0.386 & 0.338 & 0.333 & 41.9 & 0.198 & 0.453 & 0.365 & 0.353 & 27.7 & 0.215 & 0.498 & 0.375 & 0.346 & 44.7 \\
\M{1}, $S{=}2$ (1) & 0.145 & 0.338 & 0.419 & 0.427 & 133.1 & 0.170 & 0.385 & 0.419 & 0.465 & 130.6 & 0.190 & 0.435 & 0.400 & 0.465 & 122.4 \\
\midrule
\multicolumn{16}{@{}l}{\emph{1-shot direct prediction at 4\,s horizon (zero autoregressive chaining; includes \mono $S{=}50{\to}2$ reference)}} \\
\mono, $S{=}50$ (49) & 0.223 & 0.553 & 0.345 & 0.323 & 16.5 & 0.287 & 0.703 & 0.413 & 0.374 & 18.9 & 0.335 & 0.834 & 0.458 & 0.405 & 28.5 \\
\mono, $S{=}5$ (4) & 0.184 & 0.442 & 0.326 & 0.310 & 20.5 & 0.244 & 0.576 & 0.392 & 0.369 & 21.7 & 0.296 & 0.702 & 0.444 & 0.397 & 33.3 \\
\mono, $S{=}3$ (2) & 0.160 & 0.379 & 0.323 & 0.319 & 32.7 & 0.213 & 0.489 & 0.383 & 0.376 & 25.1 & 0.268 & 0.615 & 0.439 & 0.406 & 49.9 \\
\mono, $S{=}2$ (1) & 0.140 & 0.327 & 0.400 & 0.408 & 112.2 & 0.181 & 0.408 & 0.448 & 0.485 & 140.3 & 0.239 & 0.536 & 0.473 & 0.526 & 146.4 \\
\midrule
\M{1}, $S{=}50$ (49) & 0.235 & 0.582 & 0.362 & 0.343 & 19.1 & 0.295 & 0.722 & 0.422 & 0.385 & 20.3 & 0.334 & 0.828 & 0.456 & 0.399 & 31.1 \\
\M{1}, $S{=}5$ (4) & 0.192 & 0.458 & 0.344 & 0.331 & 24.7 & 0.249 & 0.583 & 0.401 & 0.382 & 25.0 & 0.289 & 0.679 & 0.440 & 0.389 & 36.4 \\
\M{1}, $S{=}3$ (2) & 0.168 & 0.393 & 0.346 & 0.344 & 44.7 & 0.218 & 0.496 & 0.393 & 0.389 & 31.0 & 0.259 & 0.590 & 0.433 & 0.401 & 55.1 \\
\M{1}, $S{=}2$ (1) & 0.148 & 0.346 & 0.438 & 0.442 & 141.8 & 0.186 & 0.419 & 0.469 & 0.510 & 172.3 & 0.229 & 0.515 & 0.476 & 0.547 & 169.7 \\


==> tab/gen/supp_b2_cal_body.tex <==
\monoat{50} & 49 & $2.154\pm0.023$ & $0.612\pm0.010$\sig & $-0.087$\sig \ci{$-0.173$, $-0.001$} & 1.56 & 1.80 & 2.06 & 3.19 & 1.42 / 1.41 \\
\at{4}{50} & 49 & $2.209\pm0.059$ & $0.617\pm0.011$\sig & $-0.032$ \ci{$-0.120$, $+0.055$} & 1.62 & 1.86 & 2.13 & 3.22 & 1.47 / 1.44 \\
\at{1}{50} & 49 & $2.229\pm0.037$ & $0.619\pm0.007$\sig & $-0.012$ \ci{$-0.101$, $+0.077$} & 1.71 & 1.86 & 2.13 & 3.22 & 1.53 / 1.41 \\
Standalone \M{0}@50 & 49 & $2.348\pm0.042$ & $0.634\pm0.009$\sig & $+0.107$\sig \ci{$+0.023$, $+0.193$} & 1.77 & 1.95 & 2.28 & 3.39 & 1.59 / 1.49 \\
\midrule
\monoat{5} & 4 & $2.091\pm0.041$ & $0.601\pm0.002$ & $-0.150$\sig$^{\ddagger}$ \ci{$-0.240$, $-0.061$} & 1.54 & 1.76 & 1.96 & 3.11 & 1.38 / 1.37 \\
\at{4}{5} & 4 & $2.100\pm0.045$ & $0.600\pm0.006$ & $-0.141$\sig$^{\ddagger}$ \ci{$-0.228$, $-0.054$} & 1.50 & 1.73 & 2.02 & 3.15 & 1.40 / 1.36 \\
\at{1}{5} & 4 & $2.130\pm0.041$ & $0.606\pm0.004$\sig & $-0.111$\sig \ci{$-0.205$, $-0.020$} & 1.52 & 1.80 & 2.07 & 3.13 & 1.45 / 1.36 \\
Standalone \M{0}@5 & 4 & $2.244\pm0.052$ & $0.622\pm0.008$\sig & $+0.004$ \ci{$-0.089$, $+0.094$} & 1.68 & 1.86 & 2.15 & 3.29 & 1.52 / 1.43 \\
\midrule
\mono Heun@3 & 4 & $2.131\pm0.020$ & $0.600\pm0.012$ & $-0.110$\sig \ci{$-0.202$, $-0.020$} & 1.61 & 1.80 & 2.04 & 3.08 & 1.44 / 1.37 \\
\mono Midpoint@3 & 4 & $2.161\pm0.031$ & $0.606\pm0.009$\sig & $-0.080$ \ci{$-0.169$, $+0.011$} & 1.63 & 1.84 & 2.04 & 3.13 & 1.43 / 1.41 \\
\M{1} Heun@3 & 4 & $2.204\pm0.043$ & $0.611\pm0.012$\sig & $-0.037$ \ci{$-0.131$, $+0.058$} & 1.66 & 1.87 & 2.13 & 3.16 & 1.54 / 1.35 \\
\M{1} Midpoint@3 & 4 & $2.153\pm0.064$ & $0.603\pm0.009$ & $-0.088$ \ci{$-0.182$, $+0.008$} & 1.57 & 1.78 & 2.10 & 3.16 & 1.48 / 1.35 \\
\midrule
\monoat{3} & 2 & $2.084\pm0.017$ & $0.601\pm0.008$ & $-0.157$\sig$^{\ddagger}$ \ci{$-0.251$, $-0.065$} & 1.48 & 1.79 & 2.01 & 3.06 & 1.40 / 1.34 \\
\at{4}{3} & 2 & $2.106\pm0.011$ & $0.604\pm0.005$\sig & $-0.135$\sig$^{\ddagger}$ \ci{$-0.226$, $-0.045$} & 1.48 & 1.76 & 2.11 & 3.08 & 1.44 / 1.32 \\
\at{1}{3} & 2 & $2.142\pm0.044$ & $0.613\pm0.006$\sig & $-0.099$\sig \ci{$-0.192$, $-0.007$} & 1.52 & 1.79 & 2.14 & 3.13 & 1.50 / 1.31 \\
\midrule
$2{\times}\monoat{3}$ & 2$\times$2 & $2.057\pm0.038$ & $0.600\pm0.008$ & $-0.184$\sig$^{\ddagger}$ \ci{$-0.281$, $-0.087$} & 1.46 & 1.79 & 1.95 & 3.02 & 1.39 / 1.32 \\
$2{\times}\at{4}{3}$ & 2$\times$2 & $2.079\pm0.028$ & $0.600\pm0.008$ & $-0.162$\sig$^{\ddagger}$ \ci{$-0.253$, $-0.071$} & 1.47 & 1.75 & 2.06 & 3.04 & 1.44 / 1.29 \\
$2{\times}\at{1}{3}$ & 2$\times$2 & $2.092\pm0.029$ & $0.602\pm0.003$ & $-0.149$\sig$^{\ddagger}$ \ci{$-0.244$, $-0.055$} & 1.48 & 1.78 & 2.04 & 3.07 & 1.45 / 1.30 \\
\midrule
\monoat{2} & 1 & $2.182\pm0.018$ & $0.620\pm0.004$\sig & $-0.059$ \ci{$-0.162$, $+0.041$} & 1.65 & 1.99 & 1.99 & 3.09 & 1.53 / 1.32 \\
\at{4}{2} & 1 & $2.138\pm0.038$ & $0.610\pm0.008$\sig & $-0.103$\sig \ci{$-0.198$, $-0.007$} & 1.58 & 1.81 & 2.08 & 3.09 & 1.54 / 1.25 \\
\at{1}{2} & 1 & $2.249\pm0.023$ & $0.631\pm0.003$\sig & $+0.008$ \ci{$-0.093$, $+0.107$} & 1.70 & 1.92 & 2.15 & 3.23 & 1.65 / 1.28 \\
\midrule
$4{\times}\monoat{2}$ & 4$\times$1 & $2.198\pm0.010$ & $0.621\pm0.006$\sig & $-0.043$ \ci{$-0.144$, $+0.056$} & 1.67 & 1.97 & 2.04 & 3.11 & 1.56 / 1.32 \\
$4{\times}\at{4}{2}$ & 4$\times$1 & $2.142\pm0.037$ & $0.609\pm0.004$\sig & $-0.099$\sig \ci{$-0.194$, $-0.005$} & 1.58 & 1.82 & 2.07 & 3.11 & 1.54 / 1.26 \\
$4{\times}\at{1}{2}$ & 4$\times$1 & $2.253\pm0.039$ & $0.632\pm0.004$\sig & $+0.013$ \ci{$-0.087$, $+0.111$} & 1.68 & 1.95 & 2.18 & 3.20 & 1.65 / 1.28 \\
\midrule
Straight line (train-fit $v_0{=}0.896$) & -- & 2.241 & 0.585 & -- & 1.19 & 1.65 & 2.31 & 3.82 & 1.60 / 1.28 \\
\cem prior mean (calibrated) & -- & 2.241 & 0.585 & -- & 1.19 & 1.65 & 2.31 & 3.82 & 1.60 / 1.28 \\
Random shooting (calibrated) & -- & 2.800 & 0.737 & -- & 2.08 & 2.31 & 2.75 & 4.06 & 1.92 / 1.72 \\
Oracle (mean of 3 best of 120) & -- & 0.690 & 0.384 & -- & 0.47 & 0.53 & 0.63 & 1.13 & 0.46 / 0.48 \\


==> tab/gen/supp_calibration_body.tex <==
Zero motion & 5.081 & 5.161 & 4.930 \\
\cem prior mean (straight line) & 1.637 & 3.780 & 0.834 \\
Straight line at train-split mean progress (one scalar) & 1.589 & 2.241 & 0.834 \\
\midrule
Random shooting (mean of 3 random candidates; 20 repetitions) & 1.77 & 4.07 & 1.08 \\
Oracle: best fresh candidate & 0.617 $\pm$ 0.005 & 1.186 $\pm$ 0.014 & 0.334 $\pm$ 0.004 \\
Oracle: mean of the 3 best fresh candidates & 0.61 & 1.08 & 0.27 \\
\midrule
\monoat{50} & 1.351 & 2.847 & 1.012 \\
\at{1}{50} & 1.371 & 2.777 & 1.014 \\
\monoat{5} & 1.294 & 2.777 & 1.007 \\
\at{4}{5} & 1.270 & 2.712 & 0.997 \\
\at{1}{5} & 1.259 & 2.676 & 1.000 \\


==> tab/gen/supp_cluster_body.tex <==
\M{1} $-$ \mono & 50 & \recon & $+0.020$ & [$-0.021$, $+0.065$] & [$-0.023$, $+0.060$] & 391 \\
\M{1} $-$ \mono & 50 & \sacson & $-0.070$ & [$-0.163$, $+0.015$] & [$-0.169$, $+0.025$] & 202 \\
\M{1} $-$ \mono & 50 & \scand & $+0.002$ & [$-0.038$, $+0.042$] & [$-0.042$, $+0.047$] & 43 \\
\midrule
\M{4} $-$ \mono & 50 & \recon & $+0.025$ & [$-0.016$, $+0.067$] & [$-0.019$, $+0.068$] & 391 \\
\M{4} $-$ \mono & 50 & \sacson & $-0.042$ & [$-0.131$, $+0.048$] & [$-0.125$, $+0.046$] & 202 \\
\M{4} $-$ \mono & 50 & \scand & $+0.012$ & [$-0.025$, $+0.052$] & [$-0.031$, $+0.054$] & 43 \\
\midrule
\M{1} $-$ \M{4} & 50 & \recon & $-0.005$ & [$-0.043$, $+0.032$] & [$-0.040$, $+0.031$] & 391 \\
\M{1} $-$ \M{4} & 50 & \sacson & $-0.028$ & [$-0.103$, $+0.044$] & [$-0.105$, $+0.049$] & 202 \\
\M{1} $-$ \M{4} & 50 & \scand & $-0.010$ & [$-0.047$, $+0.026$] & [$-0.049$, $+0.026$] & 43 \\
\midrule
\M{1} $-$ \mono & 5 & \recon & $-0.035$ & [$-0.076$, $+0.003$] & [$-0.074$, $+0.004$] & 391 \\
\M{1} $-$ \mono & 5 & \sacson & $-0.101$ & [$-0.187$, $-0.015$] & [$-0.190$, $-0.013$] & 202 \\
\M{1} $-$ \mono & 5 & \scand & $-0.007$ & [$-0.051$, $+0.036$] & [$-0.054$, $+0.035$] & 43 \\
\midrule
\M{4} $-$ \mono & 5 & \recon & $-0.024$ & [$-0.063$, $+0.013$] & [$-0.062$, $+0.016$] & 391 \\
\M{4} $-$ \mono & 5 & \sacson & $-0.065$ & [$-0.156$, $+0.021$] & [$-0.150$, $+0.022$] & 202 \\
\M{4} $-$ \mono & 5 & \scand & $-0.010$ & [$-0.052$, $+0.032$] & [$-0.057$, $+0.031$] & 43 \\
\midrule
\M{1} $-$ \M{4} & 5 & \recon & $-0.011$ & [$-0.041$, $+0.021$] & [$-0.041$, $+0.021$] & 391 \\
\M{1} $-$ \M{4} & 5 & \sacson & $-0.036$ & [$-0.105$, $+0.035$] & [$-0.106$, $+0.033$] & 202 \\
\M{1} $-$ \M{4} & 5 & \scand & $+0.003$ & [$-0.033$, $+0.038$] & [$-0.038$, $+0.045$] & 43 \\
\midrule
\M{1} $-$ \mono & 3 & \recon & $-0.028$ & [$-0.065$, $+0.008$] & [$-0.066$, $+0.010$] & 391 \\
\M{1} $-$ \mono & 3 & \sacson & $-0.056$ & [$-0.150$, $+0.034$] & [$-0.150$, $+0.036$] & 202 \\
\M{1} $-$ \mono & 3 & \scand & $-0.061$ & [$-0.104$, $-0.016$] & [$-0.105$, $-0.019$] & 43 \\
\midrule
\M{4} $-$ \mono & 3 & \recon & $-0.021$ & [$-0.054$, $+0.011$] & [$-0.055$, $+0.013$] & 391 \\
\M{4} $-$ \mono & 3 & \sacson & $-0.037$ & [$-0.129$, $+0.056$] & [$-0.148$, $+0.064$] & 202 \\
\M{4} $-$ \mono & 3 & \scand & $-0.068$ & [$-0.113$, $-0.022$] & [$-0.109$, $-0.025$] & 43 \\
\midrule
\M{1} $-$ \M{4} & 3 & \recon & $-0.007$ & [$-0.038$, $+0.023$] & [$-0.039$, $+0.024$] & 391 \\
\M{1} $-$ \M{4} & 3 & \sacson & $-0.019$ & [$-0.091$, $+0.049$] & [$-0.093$, $+0.056$] & 202 \\
\M{1} $-$ \M{4} & 3 & \scand & $+0.007$ & [$-0.025$, $+0.038$] & [$-0.017$, $+0.037$] & 43 \\
\midrule
\at{1}{5} $-$ \at{1}{50} & 5/50 & \recon & $-0.112$ & [$-0.154$, $-0.072$] & [$-0.155$, $-0.073$] & 391 \\
\at{1}{5} $-$ \at{1}{50} & 5/50 & \sacson & $-0.101$ & [$-0.172$, $-0.023$] & [$-0.181$, $-0.017$] & 202 \\
\at{1}{5} $-$ \at{1}{50} & 5/50 & \scand & $-0.014$ & [$-0.053$, $+0.025$] & [$-0.054$, $+0.031$] & 43 \\
\midrule
\monoat{5} $-$ \monoat{50} & 5/50 & \recon & $-0.057$ & [$-0.097$, $-0.016$] & [$-0.095$, $-0.022$] & 391 \\
\monoat{5} $-$ \monoat{50} & 5/50 & \sacson & $-0.070$ & [$-0.149$, $+0.008$] & [$-0.148$, $+0.011$] & 202 \\
\monoat{5} $-$ \monoat{50} & 5/50 & \scand & $-0.004$ & [$-0.040$, $+0.029$] & [$-0.041$, $+0.033$] & 43 \\


==> tab/gen/supp_difficulty_body.tex <==
\recon & near prior & 1.025 & 1.045 & 0.991 & 0.982 & $-0.035$\sig [$-0.066$, $-0.005$] & $-0.053$\sig [$-0.084$, $-0.021$] & $-0.063$\sig [$-0.102$, $-0.023$] \\
 & far from prior & 2.249 & 1.681 & 1.600 & 1.551 & $-0.168$\sig [$-0.206$, $-0.129$] & $-0.081$\sig [$-0.115$, $-0.050$] & $-0.130$\sig [$-0.173$, $-0.087$] \\
\midrule
\sacson & near prior & 2.325 & 1.669 & 1.603 & 1.600 & $-0.076$\sig [$-0.133$, $-0.013$] & $-0.066$\sig [$-0.120$, $-0.015$] & $-0.069$\sig [$-0.140$, $-0.004$] \\
 & far from prior & 5.234 & 4.006 & 3.910 & 3.897 & $-0.099$\sig [$-0.179$, $-0.022$] & $-0.096$\sig [$-0.176$, $-0.019$] & $-0.109$\sig [$-0.213$, $-0.010$] \\
\midrule
\scand & near prior & 0.371 & 0.670 & 0.676 & 0.661 & $-0.012$ [$-0.039$, $+0.016$] & $+0.006$ [$-0.019$, $+0.032$] & $-0.009$ [$-0.037$, $+0.020$] \\
 & far from prior & 1.297 & 1.405 & 1.387 & 1.360 & $-0.018$ [$-0.053$, $+0.017$] & $-0.018$ [$-0.054$, $+0.016$] & $-0.045$\sig [$-0.086$, $-0.004$] \\


==> tab/gen/supp_e12_body.tex <==
\multicolumn{7}{@{}l}{\emph{\paper \M{1} ($500$ items per dataset)}} \\
$S{=}20 - S{=}50$ (19 vs.\ 49 NFEs) & $-0.027$ [$-0.053$, $+0.001$] & $-0.021$\sig [$-0.037$, $-0.005$] & $+0.013$ [$-0.028$, $+0.059$] & $-0.002$ [$-0.027$, $+0.028$] & $+0.002$ [$-0.026$, $+0.028$] & $+0.010$ [$-0.004$, $+0.026$] \\
$S{=}10 - S{=}50$ (9 vs.\ 49 NFEs) & $-0.052$\sig [$-0.082$, $-0.020$] & $-0.056$\sig [$-0.076$, $-0.036$] & $-0.036$ [$-0.091$, $+0.025$] & $-0.060$\sig [$-0.094$, $-0.022$] & $-0.022$ [$-0.056$, $+0.010$] & $-0.010$ [$-0.030$, $+0.008$] \\
$S{=}4 - S{=}5$ (3 vs.\ 4 NFEs) & $+0.009$ [$-0.014$, $+0.033$] & $-0.004$ [$-0.019$, $+0.009$] & $-0.010$ [$-0.067$, $+0.044$] & $-0.035$ [$-0.066$, $+0.000$] & $+0.001$ [$-0.029$, $+0.030$] & $-0.003$ [$-0.018$, $+0.012$] \\
$S{=}4 - S{=}3$ (3 vs.\ 2 NFEs) & $+0.025$ [$-0.001$, $+0.052$] & $+0.015$ [$-0.000$, $+0.031$] & $-0.007$ [$-0.064$, $+0.048$] & $-0.001$ [$-0.040$, $+0.035$] & $-0.012$ [$-0.045$, $+0.018$] & $+0.010$ [$-0.007$, $+0.029$] \\
$S{=}10 - S{=}5$ (9 vs.\ 4 NFEs) & $+0.060$\sig [$+0.028$, $+0.092$] & $+0.045$\sig [$+0.029$, $+0.064$] & $+0.065$\sig [$+0.000$, $+0.130$] & $+0.027$ [$-0.012$, $+0.065$] & $-0.009$ [$-0.044$, $+0.028$] & $+0.006$ [$-0.014$, $+0.025$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ shifted Euler ($S{=}5$, 4 NFEs) & $+0.016$ [$-0.022$, $+0.056$] & $+0.016$ [$-0.007$, $+0.040$] & $+0.025$ [$-0.056$, $+0.117$] & $-0.015$ [$-0.069$, $+0.049$] & $-0.009$ [$-0.047$, $+0.031$] & $-0.008$ [$-0.029$, $+0.014$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ unif.\ Heun ($\alpha{=}1$, 4 NFEs) & $-0.058$\sig [$-0.094$, $-0.025$] & $-0.054$\sig [$-0.075$, $-0.033$] & $-0.045$ [$-0.111$, $+0.026$] & $-0.019$ [$-0.057$, $+0.020$] & $-0.019$ [$-0.052$, $+0.016$] & $-0.022$\sig [$-0.041$, $-0.001$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ unif.\ midpoint ($\alpha{=}1$, 4 NFEs) & $-0.085$\sig [$-0.122$, $-0.045$] & $-0.092$\sig [$-0.115$, $-0.069$] & $-0.048$ [$-0.120$, $+0.027$] & $-0.011$ [$-0.051$, $+0.032$] & $-0.020$ [$-0.060$, $+0.019$] & $-0.025$\sig [$-0.047$, $-0.004$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{\mono ($500$ items per dataset)}} \\
$S{=}20 - S{=}50$ (19 vs.\ 49 NFEs) & $-0.002$ [$-0.027$, $+0.026$] & $-0.012$ [$-0.028$, $+0.003$] & $+0.002$ [$-0.046$, $+0.049$] & $-0.021$ [$-0.050$, $+0.007$] & $+0.015$ [$-0.008$, $+0.038$] & $+0.009$ [$-0.005$, $+0.021$] \\
$S{=}10 - S{=}50$ (9 vs.\ 49 NFEs) & $-0.026$ [$-0.058$, $+0.007$] & $-0.033$\sig [$-0.052$, $-0.013$] & $-0.047$ [$-0.114$, $+0.005$] & $-0.064$\sig [$-0.098$, $-0.029$] & $-0.016$ [$-0.045$, $+0.010$] & $-0.009$ [$-0.027$, $+0.009$] \\
$S{=}4 - S{=}5$ (3 vs.\ 4 NFEs) & $-0.007$ [$-0.037$, $+0.020$] & $-0.011$ [$-0.026$, $+0.004$] & $-0.059$\sig [$-0.111$, $-0.006$] & $-0.059$\sig [$-0.090$, $-0.026$] & $+0.031$\sig [$+0.007$, $+0.055$] & $+0.001$ [$-0.013$, $+0.016$] \\
$S{=}4 - S{=}3$ (3 vs.\ 2 NFEs) & $+0.016$ [$-0.012$, $+0.043$] & $+0.013$ [$-0.004$, $+0.031$] & $-0.011$ [$-0.071$, $+0.048$] & $+0.036$ [$-0.001$, $+0.072$] & $-0.037$\sig [$-0.068$, $-0.003$] & $-0.025$\sig [$-0.043$, $-0.007$] \\
$S{=}10 - S{=}5$ (9 vs.\ 4 NFEs) & $+0.031$\sig [$+0.003$, $+0.060$] & $+0.035$\sig [$+0.016$, $+0.053$] & $+0.023$ [$-0.051$, $+0.092$] & $+0.017$ [$-0.028$, $+0.057$] & $-0.012$ [$-0.041$, $+0.018$] & $-0.003$ [$-0.020$, $+0.016$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ shifted Euler ($S{=}5$, 4 NFEs) & $+0.008$ [$-0.027$, $+0.043$] & $+0.013$ [$-0.015$, $+0.039$] & $-0.029$ [$-0.109$, $+0.056$] & $-0.071$\sig [$-0.118$, $-0.019$] & $+0.001$ [$-0.035$, $+0.036$] & $+0.006$ [$-0.015$, $+0.028$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ unif.\ Heun ($\alpha{=}1$, 4 NFEs) & $-0.041$\sig [$-0.074$, $-0.010$] & $-0.045$\sig [$-0.067$, $-0.023$] & $+0.015$ [$-0.052$, $+0.079$] & $-0.028$ [$-0.068$, $+0.006$] & $+0.001$ [$-0.029$, $+0.030$] & $-0.002$ [$-0.020$, $+0.017$] \\
Unif.\ Euler ($\alpha{=}1$) $-$ unif.\ midpoint ($\alpha{=}1$, 4 NFEs) & $-0.064$\sig [$-0.099$, $-0.029$] & $-0.078$\sig [$-0.103$, $-0.056$] & $-0.046$ [$-0.112$, $+0.021$] & $-0.042$ [$-0.084$, $+0.001$] & $-0.032$\sig [$-0.062$, $-0.002$] & $-0.010$ [$-0.030$, $+0.010$] \\


==> tab/gen/supp_gen_full_body.tex <==
\M{1} & 50 & 0.385 & 0.422 & 20.3 & 0.343 & 0.362 & 19.1 & 0.399 & 0.456 & 31.1 \\
 & 20 & 0.383 & 0.418 & 21.3 & 0.340 & 0.358 & 19.1 & 0.396 & 0.453 & 31.5 \\
 & 10 & 0.382 & 0.412 & 22.7 & 0.335 & 0.352 & 20.1 & 0.393 & 0.448 & 32.5 \\
 & 7 & 0.382 & 0.407 & 23.7 & 0.333 & 0.348 & 21.4 & 0.391 & 0.444 & 33.7 \\
 & 5 & 0.382 & 0.401 & 25.0 & 0.331 & 0.344 & 24.7 & 0.389 & 0.440 & 36.4 \\
 & 4 & 0.383 & 0.396 & 26.4 & 0.333 & 0.342 & 29.5 & 0.390 & 0.436 & 40.5 \\
 & 3 & 0.389 & 0.393 & 31.0 & 0.344 & 0.346 & 44.7 & 0.401 & 0.433 & 55.1 \\
 & 2 & 0.510 & 0.469 & 172.5 & 0.442 & 0.438 & 142.0 & 0.547 & 0.476 & 169.7 \\
\midrule
\M{2} & 50 & 0.382 & 0.420 & 19.6 & 0.340 & 0.358 & 18.2 & 0.399 & 0.456 & 30.5 \\
 & 20 & 0.380 & 0.416 & 20.5 & 0.336 & 0.354 & 18.3 & 0.396 & 0.453 & 30.8 \\
 & 10 & 0.379 & 0.410 & 21.7 & 0.332 & 0.348 & 19.3 & 0.393 & 0.447 & 31.6 \\
 & 5 & 0.379 & 0.399 & 23.6 & 0.327 & 0.340 & 23.6 & 0.389 & 0.439 & 35.4 \\
 & 3 & 0.387 & 0.390 & 29.0 & 0.338 & 0.341 & 41.9 & 0.400 & 0.432 & 53.8 \\
\midrule
\M{3} & 50 & 0.381 & 0.419 & 19.4 & 0.336 & 0.356 & 17.6 & 0.399 & 0.455 & 29.6 \\
 & 20 & 0.379 & 0.415 & 20.2 & 0.332 & 0.352 & 17.7 & 0.396 & 0.452 & 29.9 \\
 & 10 & 0.378 & 0.409 & 21.3 & 0.328 & 0.346 & 18.6 & 0.393 & 0.447 & 30.6 \\
 & 5 & 0.377 & 0.397 & 23.3 & 0.324 & 0.337 & 22.5 & 0.389 & 0.438 & 34.4 \\
 & 3 & 0.384 & 0.388 & 27.9 & 0.333 & 0.337 & 39.3 & 0.398 & 0.431 & 52.8 \\
\midrule
\M{4} & 50 & 0.379 & 0.418 & 19.1 & 0.333 & 0.354 & 17.1 & 0.399 & 0.455 & 29.1 \\
 & 20 & 0.378 & 0.414 & 20.0 & 0.330 & 0.349 & 17.3 & 0.397 & 0.451 & 29.4 \\
 & 10 & 0.376 & 0.408 & 20.8 & 0.326 & 0.344 & 18.2 & 0.393 & 0.446 & 30.3 \\
 & 7 & 0.376 & 0.403 & 21.8 & 0.323 & 0.340 & 19.2 & 0.391 & 0.442 & 31.5 \\
 & 5 & 0.375 & 0.397 & 22.9 & 0.320 & 0.335 & 21.6 & 0.389 & 0.438 & 34.1 \\
 & 4 & 0.376 & 0.392 & 24.2 & 0.320 & 0.332 & 25.3 & 0.388 & 0.434 & 37.8 \\
 & 3 & 0.382 & 0.387 & 27.6 & 0.329 & 0.334 & 37.1 & 0.398 & 0.431 & 52.1 \\
 & 2 & 0.495 & 0.457 & 154.1 & 0.422 & 0.416 & 124.8 & 0.537 & 0.471 & 163.6 \\
\midrule
\mono & 50 & 0.374 & 0.413 & 18.9 & 0.323 & 0.345 & 16.5 & 0.405 & 0.458 & 28.5 \\
 & 20 & 0.372 & 0.409 & 19.3 & 0.320 & 0.341 & 16.7 & 0.403 & 0.455 & 28.9 \\
 & 10 & 0.370 & 0.403 & 20.1 & 0.316 & 0.335 & 17.4 & 0.401 & 0.451 & 29.8 \\
 & 7 & 0.370 & 0.398 & 20.7 & 0.313 & 0.331 & 18.5 & 0.399 & 0.448 & 30.9 \\
 & 5 & 0.369 & 0.392 & 21.7 & 0.310 & 0.326 & 20.5 & 0.397 & 0.444 & 33.3 \\
 & 4 & 0.370 & 0.387 & 22.7 & 0.310 & 0.323 & 23.3 & 0.397 & 0.441 & 36.8 \\
 & 3 & 0.376 & 0.383 & 25.1 & 0.319 & 0.323 & 32.7 & 0.406 & 0.439 & 49.9 \\
 & 2 & 0.485 & 0.448 & 140.5 & 0.408 & 0.400 & 112.4 & 0.526 & 0.473 & 146.4 \\
\midrule
\mono, naive \M{1} slice & 50 & 0.939 & 0.866 & 494.2 & 0.873 & 0.847 & 408.0 & 0.933 & 0.889 & 444.3 \\
 & 5 & 0.795 & 0.877 & 432.5 & 0.825 & 0.859 & 442.3 & 0.900 & 0.887 & 439.1 \\
\midrule
Standalone \M{1} & 50 & 0.381 & 0.418 & 20.3 & 0.334 & 0.354 & 17.7 & 0.401 & 0.457 & 30.1 \\
 & 5 & 0.378 & 0.397 & 23.9 & 0.322 & 0.336 & 22.7 & 0.392 & 0.440 & 35.8 \\
\midrule
Standalone \M{0} & 50 & 0.399 & 0.432 & 21.3 & 0.358 & 0.374 & 20.9 & 0.408 & 0.465 & 33.6 \\
 & 5 & 0.397 & 0.411 & 26.2 & 0.345 & 0.358 & 27.4 & 0.398 & 0.448 & 41.1 \\


==> tab/gen/supp_gen_horizon_body.tex <==
\recon & \M{1} & 50 & 0.350 & 0.366 & 0.385 & 0.407 & 0.460 & 19.0 & 19.5 & 20.3 & 21.3 & 20.3 \\
\recon & \M{1} & 5 & 0.346 & 0.362 & 0.382 & 0.406 & 0.463 & 23.2 & 24.0 & 25.0 & 26.5 & 25.0 \\
\recon & \M{2} & 50 & 0.348 & 0.363 & 0.382 & 0.404 & 0.458 & 18.5 & 18.8 & 19.6 & 20.5 & 19.7 \\
\recon & \M{2} & 5 & 0.343 & 0.360 & 0.379 & 0.403 & 0.460 & 22.4 & 22.8 & 23.6 & 25.0 & 23.9 \\
\recon & \M{3} & 50 & 0.346 & 0.362 & 0.381 & 0.403 & 0.458 & 18.2 & 18.6 & 19.4 & 20.4 & 19.3 \\
\recon & \M{3} & 5 & 0.341 & 0.358 & 0.377 & 0.401 & 0.459 & 21.8 & 22.4 & 23.3 & 24.2 & 23.2 \\
\recon & \M{4} & 50 & 0.345 & 0.361 & 0.379 & 0.402 & 0.457 & 17.9 & 18.1 & 19.1 & 20.0 & 19.1 \\
\recon & \M{4} & 5 & 0.340 & 0.356 & 0.375 & 0.400 & 0.458 & 21.5 & 21.9 & 22.9 & 23.9 & 22.9 \\
\recon & \mono & 50 & 0.341 & 0.356 & 0.374 & 0.396 & 0.452 & 18.0 & 18.1 & 18.9 & 19.3 & 18.4 \\
\recon & \mono & 5 & 0.335 & 0.350 & 0.369 & 0.394 & 0.453 & 20.7 & 21.2 & 21.7 & 22.7 & 21.8 \\
\recon & Standalone \M{1} & 50 & 0.348 & 0.363 & 0.381 & 0.404 & 0.458 & 19.3 & 19.7 & 20.3 & 20.7 & 20.2 \\
\recon & Standalone \M{1} & 5 & 0.344 & 0.359 & 0.378 & 0.402 & 0.460 & 22.7 & 23.3 & 23.9 & 24.7 & 23.8 \\
\recon & Standalone \M{0} & 50 & 0.368 & 0.383 & 0.399 & 0.420 & 0.472 & 19.9 & 20.4 & 21.3 & 22.3 & 21.2 \\
\recon & Standalone \M{0} & 5 & 0.366 & 0.380 & 0.397 & 0.419 & 0.471 & 23.9 & 24.7 & 26.2 & 27.2 & 26.3 \\
\midrule
\sacson & \M{1} & 50 & 0.332 & 0.339 & 0.343 & 0.348 & 0.379 & 18.8 & 18.9 & 19.1 & 19.4 & 21.0 \\
\sacson & \M{1} & 5 & 0.321 & 0.328 & 0.331 & 0.335 & 0.365 & 24.0 & 24.2 & 24.7 & 24.9 & 26.6 \\
\sacson & \M{2} & 50 & 0.329 & 0.336 & 0.340 & 0.345 & 0.375 & 17.9 & 18.0 & 18.2 & 18.6 & 20.1 \\
\sacson & \M{2} & 5 & 0.318 & 0.324 & 0.327 & 0.332 & 0.361 & 23.0 & 23.2 & 23.6 & 23.8 & 25.5 \\
\sacson & \M{3} & 50 & 0.326 & 0.333 & 0.336 & 0.341 & 0.371 & 17.1 & 17.2 & 17.6 & 17.9 & 19.2 \\
\sacson & \M{3} & 5 & 0.314 & 0.320 & 0.324 & 0.328 & 0.358 & 21.8 & 22.1 & 22.5 & 22.8 & 24.6 \\
\sacson & \M{4} & 50 & 0.323 & 0.330 & 0.333 & 0.338 & 0.369 & 16.8 & 16.9 & 17.1 & 17.5 & 18.7 \\
\sacson & \M{4} & 5 & 0.311 & 0.317 & 0.320 & 0.325 & 0.355 & 21.1 & 21.3 & 21.6 & 22.1 & 23.7 \\
\sacson & \mono & 50 & 0.314 & 0.319 & 0.323 & 0.328 & 0.361 & 16.1 & 16.4 & 16.5 & 16.8 & 17.8 \\
\sacson & \mono & 5 & 0.302 & 0.307 & 0.310 & 0.315 & 0.347 & 20.3 & 20.5 & 20.5 & 20.9 & 22.4 \\
\sacson & Standalone \M{1} & 50 & 0.325 & 0.331 & 0.334 & 0.340 & 0.371 & 17.2 & 17.4 & 17.7 & 17.9 & 19.5 \\
\sacson & Standalone \M{1} & 5 & 0.313 & 0.319 & 0.322 & 0.327 & 0.357 & 22.0 & 22.2 & 22.7 & 23.0 & 24.8 \\
\sacson & Standalone \M{0} & 50 & 0.349 & 0.355 & 0.358 & 0.364 & 0.392 & 20.5 & 21.1 & 20.9 & 21.5 & 23.4 \\
\sacson & Standalone \M{0} & 5 & 0.337 & 0.342 & 0.345 & 0.349 & 0.376 & 27.1 & 27.2 & 27.4 & 27.7 & 30.2 \\
\midrule
\scand & \M{1} & 50 & 0.349 & 0.373 & 0.399 & 0.428 & 0.459 & 27.1 & 28.5 & 31.1 & 33.0 & 35.6 \\
\scand & \M{1} & 5 & 0.337 & 0.362 & 0.389 & 0.419 & 0.452 & 30.9 & 33.8 & 36.4 & 39.4 & 41.4 \\
\scand & \M{2} & 50 & 0.349 & 0.373 & 0.399 & 0.427 & 0.458 & 26.5 & 28.0 & 30.5 & 32.3 & 34.4 \\
\scand & \M{2} & 5 & 0.336 & 0.361 & 0.389 & 0.419 & 0.451 & 30.0 & 32.9 & 35.4 & 37.5 & 39.4 \\
\scand & \M{3} & 50 & 0.348 & 0.373 & 0.399 & 0.427 & 0.458 & 25.9 & 27.6 & 29.6 & 31.3 & 33.2 \\
\scand & \M{3} & 5 & 0.336 & 0.361 & 0.389 & 0.418 & 0.450 & 29.4 & 31.9 & 34.4 & 36.7 & 38.0 \\
\scand & \M{4} & 50 & 0.349 & 0.373 & 0.399 & 0.427 & 0.458 & 25.6 & 27.2 & 29.1 & 31.1 & 32.8 \\
\scand & \M{4} & 5 & 0.336 & 0.362 & 0.389 & 0.418 & 0.450 & 29.0 & 31.3 & 34.1 & 36.3 & 37.3 \\
\scand & \mono & 50 & 0.362 & 0.384 & 0.405 & 0.428 & 0.456 & 26.7 & 27.9 & 28.5 & 29.9 & 31.3 \\
\scand & \mono & 5 & 0.352 & 0.375 & 0.397 & 0.421 & 0.450 & 30.4 & 31.8 & 33.3 & 34.7 & 35.5 \\
\scand & Standalone \M{1} & 50 & 0.352 & 0.376 & 0.401 & 0.426 & 0.456 & 26.8 & 28.3 & 30.1 & 32.3 & 34.2 \\
\scand & Standalone \M{1} & 5 & 0.340 & 0.365 & 0.392 & 0.419 & 0.450 & 30.6 & 33.0 & 35.8 & 38.2 & 39.4 \\
\scand & Standalone \M{0} & 50 & 0.364 & 0.384 & 0.408 & 0.435 & 0.467 & 30.4 & 31.9 & 33.6 & 35.4 & 38.4 \\
\scand & Standalone \M{0} & 5 & 0.351 & 0.372 & 0.398 & 0.427 & 0.461 & 35.3 & 37.9 & 41.1 & 43.7 & 45.8 \\


==> tab/gen/supp_kernel_bench_body.tex <==
\mono & 13.18 / 12.02 & 480.6 & 196.2 & 6.70 & 213.5 & 87.2 & 4.71 & 2.25$\times$ \\
\M{4} & 15.04 / 14.04 & 482.2 & 196.9 & 6.70 & 214.7 & 87.7 & 4.71 & 2.25$\times$ \\
\M{3} & -- & 464.9 & 189.8 & 6.70 & 196.6 & 80.3 & 4.24 & 2.36$\times$ \\
\M{2} & -- & 456.1 & 186.2 & 6.70 & 187.2 & 76.5 & 4.24 & 2.44$\times$ \\
\M{1} & 14.48 / 15.40 & 451.6 & 184.4 & 6.70 & 182.4 & 74.5 & 4.24 & 2.48$\times$ \\


==> tab/gen/supp_noise_body.tex <==
100 \sacson (seed 0) & \at{4}{50} & 5 & 0.87 & 0.77 & 0.88 & 0.52 & 2.82 & 2.71 & 2.65 & 2.63 \\
100 \sacson (seed 0) & \at{4}{5} & 3 & 0.61 & 0.58 & 0.61 & 0.69 & 2.76 & 2.63 & 2.60 & -- \\
100 \sacson (seed 0) & \at{1}{5} & 3 & 0.60 & 0.58 & 0.60 & 0.69 & 2.75 & 2.54 & 2.50 & -- \\
\midrule
500 \recon (seed 0) & \at{1}{50} & 3 & 0.67 & 0.65 & 0.67 & 0.65 & 1.379 & 1.341 & 1.341 & -- \\
500 \sacson (seed 0) & \at{1}{50} & 3 & 0.83 & 0.80 & 0.90 & 0.52 & 2.818 & 2.703 & 2.636 & -- \\
\midrule
500 \recon (seeds 0--2) & \at{1}{5} & 3 & 0.48 & 0.47 & 0.46 & 0.79 & 1.278 & 1.252 & 1.247 & -- \\
500 \sacson (seeds 0--2) & \at{1}{5} & 3 & 0.61 & 0.59 & 0.62 & 0.69 & 2.754 & 2.638 & 2.592 & -- \\
500 \scand (seeds 0--2) & \at{1}{5} & 3 & 0.42 & 0.41 & 0.37 & 0.82 & 1.004 & 1.001 & 0.998 & -- \\
\midrule
500 \recon (seeds 0--2) & \at{1}{3} & 2 & 0.32 & 0.32 & 0.30 & 0.88 & 1.256 & 1.240 & -- & -- \\
500 \sacson (seeds 0--2) & \at{1}{3} & 2 & 0.43 & 0.43 & 0.44 & 0.81 & 2.719 & 2.627 & -- & -- \\
500 \scand (seeds 0--2) & \at{1}{3} & 2 & 0.31 & 0.31 & 0.27 & 0.89 & 0.988 & 1.003 & -- & -- \\
500 \recon (seeds 0--2) & \at{4}{3} & 2 & 0.32 & 0.32 & 0.30 & 0.89 & 1.250 & 1.238 & -- & -- \\
500 \sacson (seeds 0--2) & \at{4}{3} & 2 & 0.43 & 0.43 & 0.45 & 0.81 & 2.738 & 2.644 & -- & -- \\
500 \scand (seeds 0--2) & \at{4}{3} & 2 & 0.31 & 0.31 & 0.28 & 0.88 & 1.002 & 0.994 & -- & -- \\
500 \recon (seeds 0--2) & \monoat{3} & 2 & 0.34 & 0.34 & 0.33 & 0.88 & 1.277 & 1.255 & -- & -- \\
500 \sacson (seeds 0--2) & \monoat{3} & 2 & 0.41 & 0.41 & 0.42 & 0.83 & 2.667 & 2.591 & -- & -- \\
500 \scand (seeds 0--2) & \monoat{3} & 2 & 0.33 & 0.33 & 0.28 & 0.87 & 1.050 & 1.051 & -- & -- \\
\midrule
500 \recon (seeds 0--2) & \at{1}{2} & 4 & 0.10 & 0.10 & 0.10 & 0.98 & 1.251 & 1.253 & 1.256 & 1.257 \\
500 \sacson (seeds 0--2) & \at{1}{2} & 4 & 0.23 & 0.22 & 0.25 & 0.94 & 2.792 & 2.769 & 2.759 & 2.756 \\
500 \scand (seeds 0--2) & \at{1}{2} & 4 & 0.10 & 0.10 & 0.09 & 0.98 & 1.000 & 1.002 & 1.000 & 0.998 \\
500 \recon (seeds 0--2) & \monoat{2} & 4 & 0.11 & 0.11 & 0.11 & 0.98 & 1.264 & 1.263 & 1.263 & 1.263 \\
500 \sacson (seeds 0--2) & \monoat{2} & 4 & 0.22 & 0.21 & 0.24 & 0.95 & 2.691 & 2.669 & 2.661 & 2.663 \\
500 \scand (seeds 0--2) & \monoat{2} & 4 & 0.11 & 0.11 & 0.09 & 0.98 & 1.090 & 1.092 & 1.088 & 1.088 \\
\midrule
\multicolumn{11}{@{}l}{\emph{Second-order solver noise-to-signal on the nested \paper \M{1} shard (100 items/dataset, shard 0/5, seed 0)}} \\
100 \recon (shard 0/5) & \at{1}{5} (Euler, 4 NFE) & 3 & 0.48 & 0.47 & 0.46 & 0.78 & 1.279 & 1.222 & 1.210 & -- \\
100 \recon (shard 0/5) & \at{1}{3} (Euler, 2 NFE) & 2 & 0.32 & 0.32 & 0.30 & 0.88 & 1.259 & 1.205 & -- & -- \\
100 \recon (shard 0/5) & \at{1}{3} (Heun, 4 NFE) & 3 & 0.46 & 0.45 & 0.44 & 0.81 & 1.402 & 1.422 & 1.366 & -- \\
100 \recon (shard 0/5) & \at{1}{3} (midpoint, 4 NFE) & 3 & 0.54 & 0.52 & 0.53 & 0.75 & 1.370 & 1.337 & 1.321 & -- \\
\midrule
100 \sacson (shard 0/5) & \at{1}{5} (Euler, 4 NFE) & 3 & 0.62 & 0.59 & 0.63 & 0.67 & 2.587 & 2.464 & 2.428 & -- \\
100 \sacson (shard 0/5) & \at{1}{3} (Euler, 2 NFE) & 2 & 0.44 & 0.44 & 0.46 & 0.79 & 2.587 & 2.550 & -- & -- \\
100 \sacson (shard 0/5) & \at{1}{3} (Heun, 4 NFE) & 3 & 0.49 & 0.47 & 0.47 & 0.76 & 2.731 & 2.712 & 2.685 & -- \\
100 \sacson (shard 0/5) & \at{1}{3} (midpoint, 4 NFE) & 3 & 0.60 & 0.58 & 0.59 & 0.68 & 2.696 & 2.551 & 2.484 & -- \\
\midrule
100 \scand (shard 0/5) & \at{1}{5} (Euler, 4 NFE) & 3 & 0.41 & 0.40 & 0.36 & 0.83 & 1.129 & 1.167 & 1.145 & -- \\
100 \scand (shard 0/5) & \at{1}{3} (Euler, 2 NFE) & 2 & 0.31 & 0.31 & 0.27 & 0.89 & 1.107 & 1.125 & -- & -- \\
100 \scand (shard 0/5) & \at{1}{3} (Heun, 4 NFE) & 3 & 0.37 & 0.36 & 0.30 & 0.85 & 1.148 & 1.136 & 1.111 & -- \\
100 \scand (shard 0/5) & \at{1}{3} (midpoint, 4 NFE) & 3 & 0.41 & 0.40 & 0.35 & 0.83 & 1.128 & 1.143 & 1.137 & -- \\


==> tab/gen/supp_nullcal_body.tex <==
Same configuration, two seeds & 0 / 30 & 0.89 & 3 / 30 & 1.24 & 0 / 30 & 0.94 & 3 / 90 & 1.06 \\
Model difference, two seeds & 2 / 24 & 1.25 & 9 / 24 & 1.69 & 0 / 24 & 0.78 & 11 / 72 & 1.30 \\
Step-count difference, two seeds & 1 / 27 & 1.14 & 2 / 27 & 1.00 & 4 / 27 & 0.99 & 7 / 81 & 1.07 \\
\midrule
All & 3 / 81 & 1.08 & 14 / 81 & 1.36 & 4 / 81 & 1.04 & 21 / 243 & 1.17 \\


==> tab/gen/supp_plan_full_body.tex <==
All-\M{1} & 50 & 1.37 & 0.366 & 2.78 & 0.683 & 1.01 & 0.284 & 176.1 \\
 & 20 & 1.34 & 0.365 & 2.79 & 0.688 & 1.02 & 0.283 & 68.6 \\
 & 10 & 1.32 & 0.365 & 2.74 & 0.684 & 0.99 & 0.280 & 32.8 \\
 & 5 & 1.26 & 0.364 & 2.68 & 0.681 & 1.00 & 0.282 & 14.9 \\
 & 4 & 1.27 & 0.369 & 2.67 & 0.683 & 1.00 & 0.282 & 11.2 \\
 & 3 & 1.24 & 0.370 & 2.67 & 0.688 & 1.01 & 0.284 & 7.6 \\
 & 2 & 1.26 & 0.379 & 2.80 & 0.708 & 0.99 & 0.281 & 4.0 \\
\midrule
All-\M{2} & 5 & 1.26 & 0.364 & 2.71 & 0.679 & 1.01 & 0.285 & 14.9 \\
\midrule
All-\M{3} & 5 & 1.27 & 0.361 & 2.75 & 0.685 & 1.00 & 0.280 & 15.2 \\
\midrule
All-\M{4} & 50 & 1.38 & 0.371 & 2.81 & 0.686 & 1.02 & 0.284 & 188.2 \\
 & 20 & 1.34 & 0.369 & 2.82 & 0.691 & 1.01 & 0.280 & 73.2 \\
 & 10 & 1.31 & 0.366 & 2.76 & 0.680 & 1.00 & 0.280 & 34.9 \\
 & 5 & 1.27 & 0.361 & 2.71 & 0.680 & 1.00 & 0.278 & 15.7 \\
 & 3 & 1.25 & 0.367 & 2.69 & 0.684 & 1.01 & 0.282 & 8.0 \\
 & 2 & 1.25 & 0.373 & 2.76 & 0.698 & 0.99 & 0.280 & 4.2 \\
\midrule
\mono & 50 & 1.35 & 0.366 & 2.85 & 0.696 & 1.01 & 0.286 & 187.6 \\
 & 20 & 1.35 & 0.367 & 2.85 & 0.695 & 1.03 & 0.289 & 73.0 \\
 & 10 & 1.32 & 0.364 & 2.80 & 0.689 & 1.00 & 0.285 & 34.9 \\
 & 5 & 1.29 & 0.363 & 2.78 & 0.687 & 1.01 & 0.284 & 15.7 \\
 & 4 & 1.29 & 0.368 & 2.72 & 0.681 & 1.04 & 0.288 & 11.9 \\
 & 3 & 1.27 & 0.367 & 2.73 & 0.690 & 1.07 & 0.293 & 8.0 \\
 & 2 & 1.26 & 0.367 & 2.71 & 0.685 & 1.10 & 0.299 & 4.2 \\
\midrule
\mono, naive \M{1} slice & 5 & 1.73 & 0.487 & 4.86 & 1.068 & 1.09 & 0.307 & 14.8 \\


==> tab/gen/supp_pooled_body.tex <==
\multicolumn{7}{@{}l}{\emph{Granularity at a fixed step count}} \\
\M{1}@50 $-$ {\mono}@50 & $+0.020$ / $+0.022$ / $-0.028$ & $+0.005$ [$-0.021$, $+0.032$] & $-0.070$ / $+0.085$ / $-0.020$ & $-0.002$ [$-0.064$, $+0.053$] & $+0.002$ / $-0.027$ / $-0.012$ & $-0.012$ [$-0.036$, $+0.013$] \\
\M{1}@5 $-$ {\mono}@5 & $-0.035$ / $-0.054$\sig / $+0.002$ & $-0.029$\sig [$-0.054$, $-0.004$] & $-0.101$\sig / $+0.113$\sig / $-0.036$ & $-0.008$ [$-0.065$, $+0.052$] & $-0.007$ / $-0.030$ / $-0.026$ & $-0.021$ [$-0.044$, $+0.003$] \\
\M{1}@3 $-$ {\mono}@3 & $-0.028$ / $-0.038$ / $-0.006$ & $-0.024$ [$-0.049$, $+0.001$] & $-0.056$ / $+0.123$\sig / $+0.090$\sig & $+0.053$ [$-0.009$, $+0.113$] & $-0.061$\sig / $-0.077$\sig / $-0.043$\sig & $-0.060$\sig [$-0.090$, $-0.033$] \\
\M{1}@2 $-$ {\mono}@2 & $-0.002$ / $-0.027$ / $-0.017$ & $-0.015$ [$-0.044$, $+0.016$] & $+0.097$ / $+0.118$\sig / $+0.092$ & $+0.102$\sig [$+0.032$, $+0.175$] & $-0.110$\sig / $-0.088$\sig / $-0.096$\sig & $-0.098$\sig [$-0.128$, $-0.069$] \\
\M{4}@50 $-$ {\mono}@50 & $+0.025$ / $+0.007$ / $-0.025$ & $+0.002$ [$-0.023$, $+0.028$] & $-0.042$ / $+0.067$ / $-0.046$ & $-0.007$ [$-0.064$, $+0.053$] & $+0.012$ / $-0.049$\sig / $+0.009$ & $-0.009$ [$-0.033$, $+0.013$] \\
\M{4}@5 $-$ {\mono}@5 & $-0.024$ / $-0.016$ / $-0.031$ & $-0.024$ [$-0.048$, $+0.001$] & $-0.065$ / $+0.077$ / $+0.033$ & $+0.015$ [$-0.038$, $+0.071$] & $-0.010$ / $-0.041$ / $-0.028$ & $-0.027$\sig [$-0.051$, $-0.002$] \\
\M{4}@3 $-$ {\mono}@3 & $-0.021$ / $-0.038$\sig / $-0.004$ & $-0.021$ [$-0.045$, $+0.004$] & $-0.037$ / $+0.142$\sig / $+0.132$\sig & $+0.079$\sig [$+0.018$, $+0.142$] & $-0.068$\sig / $-0.062$\sig / $-0.021$ & $-0.050$\sig [$-0.081$, $-0.021$] \\
\M{4}@2 $-$ {\mono}@2 & $-0.015$ / $-0.018$ / $-0.030$ & $-0.021$ [$-0.049$, $+0.007$] & $+0.056$ / $+0.076$ / $+0.011$ & $+0.048$ [$-0.027$, $+0.120$] & $-0.104$\sig / $-0.088$\sig / $-0.095$\sig & $-0.096$\sig [$-0.124$, $-0.067$] \\
\M{1}@50 $-$ \M{4}@50 & $-0.005$ / $+0.015$ / $-0.002$ & $+0.003$ [$-0.019$, $+0.024$] & $-0.028$ / $+0.018$ / $+0.026$ & $+0.005$ [$-0.045$, $+0.051$] & $-0.010$ / $+0.022$ / $-0.021$ & $-0.003$ [$-0.023$, $+0.018$] \\
\M{1}@5 $-$ \M{4}@5 & $-0.011$ / $-0.038$\sig / $+0.033$\sig & $-0.005$ [$-0.025$, $+0.013$] & $-0.036$ / $+0.036$ / $-0.069$ & $-0.023$ [$-0.067$, $+0.021$] & $+0.003$ / $+0.011$ / $+0.002$ & $+0.006$ [$-0.016$, $+0.025$] \\
\M{1}@3 $-$ \M{4}@3 & $-0.007$ / $+0.000$ / $-0.002$ & $-0.003$ [$-0.020$, $+0.013$] & $-0.019$ / $-0.019$ / $-0.042$ & $-0.027$ [$-0.072$, $+0.015$] & $+0.007$ / $-0.014$ / $-0.023$ & $-0.010$ [$-0.029$, $+0.010$] \\
\M{1}@2 $-$ \M{4}@2 & $+0.013$ / $-0.009$ / $+0.013$ & $+0.006$ [$-0.013$, $+0.023$] & $+0.041$ / $+0.042$ / $+0.081$\sig & $+0.055$\sig [$+0.011$, $+0.099$] & $-0.006$ / $0.000$ / $-0.001$ & $-0.002$ [$-0.022$, $+0.017$] \\
Standalone \M{1}@50 $-$ \M{1}@50 & $-0.015$ / $-0.011$ / $+0.028$ & $+0.001$ [$-0.024$, $+0.026$] & $+0.048$ / $-0.070$ / $-0.003$ & $-0.008$ [$-0.058$, $+0.049$] & $-0.009$ / $-0.007$ / $+0.004$ & $-0.004$ [$-0.026$, $+0.019$] \\
Standalone \M{1}@50 $-$ {\mono}@50 & $+0.005$ / $+0.011$ / $+0.001$ & $+0.006$ [$-0.020$, $+0.034$] & $-0.022$ / $+0.014$ / $-0.022$ & $-0.010$ [$-0.062$, $+0.052$] & $-0.007$ / $-0.033$ / $-0.008$ & $-0.016$ [$-0.038$, $+0.006$] \\
Standalone \M{1}@5 $-$ \M{1}@5 & $+0.026$ / $+0.032$ / $-0.017$ & $+0.013$ [$-0.009$, $+0.036$] & $+0.017$ / $-0.100$\sig / $-0.012$ & $-0.032$ [$-0.085$, $+0.025$] & $-0.016$ / $-0.011$ / $-0.023$ & $-0.017$ [$-0.039$, $+0.005$] \\
Standalone \M{1}@5 $-$ {\mono}@5 & $-0.009$ / $-0.022$ / $-0.015$ & $-0.016$ [$-0.040$, $+0.008$] & $-0.083$ / $+0.012$ / $-0.047$ & $-0.040$ [$-0.098$, $+0.021$] & $-0.023$ / $-0.042$ / $-0.048$\sig & $-0.038$\sig [$-0.063$, $-0.011$] \\
Standalone \M{0}@50 $-$ \M{1}@5 & $+0.160$\sig / $+0.152$\sig / $+0.095$\sig & $+0.136$\sig [$+0.106$, $+0.171$] & $+0.333$\sig / $+0.173$\sig / $+0.306$\sig & $+0.271$\sig [$+0.198$, $+0.340$] & $+0.010$ / $+0.009$ / $+0.024$ & $+0.014$ [$-0.009$, $+0.040$] \\
Standalone \M{0}@5 $-$ \M{1}@5 & $+0.011$ / $+0.004$ / $-0.022$ & $-0.002$ [$-0.029$, $+0.026$] & $+0.189$\sig / $+0.084$ / $+0.231$\sig & $+0.168$\sig [$+0.094$, $+0.241$] & $-0.014$ / $+0.010$ / $-0.006$ & $-0.003$ [$-0.028$, $+0.022$] \\
Standalone \M{0}@3 $-$ \M{1}@5 & $+0.009$ / $+0.006$ / $+0.026$ & $+0.014$ [$-0.017$, $+0.042$] & $+0.194$\sig / $+0.085$ / $+0.198$\sig & $+0.159$\sig [$+0.084$, $+0.233$] & $-0.007$ / $+0.016$ / $-0.024$ & $-0.005$ [$-0.032$, $+0.021$] \\
Standalone \M{0}@2 $-$ \M{1}@2 & $+0.014$ / $+0.049$\sig / $+0.046$\sig & $+0.037$\sig [$+0.008$, $+0.066$] & $+0.105$ / $+0.141$\sig / $+0.081$ & $+0.109$\sig [$+0.022$, $+0.192$] & $+0.030$ / $+0.037$ / $-0.015$ & $+0.017$ [$-0.010$, $+0.046$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{Against the 50-step monolithic protocol}} \\
\M{1}@5 $-$ {\mono}@50 & $-0.092$\sig / $-0.112$\sig / $-0.085$\sig & $-0.096$\sig [$-0.126$, $-0.068$] & $-0.171$\sig / $+0.020$ / $-0.115$\sig & $-0.089$\sig [$-0.148$, $-0.028$] & $-0.011$ / $-0.043$\sig / $-0.027$ & $-0.027$\sig [$-0.051$, $-0.004$] \\
\M{1}@3 $-$ {\mono}@50 & $-0.108$\sig / $-0.117$\sig / $-0.122$\sig & $-0.116$\sig [$-0.149$, $-0.084$] & $-0.174$\sig / $-0.070$ / $-0.125$\sig & $-0.123$\sig [$-0.185$, $-0.053$] & $+0.002$ / $-0.075$\sig / $-0.048$\sig & $-0.040$\sig [$-0.067$, $-0.014$] \\
\M{1}@2 $-$ {\mono}@50 & $-0.090$\sig / $-0.126$\sig / $-0.124$\sig & $-0.114$\sig [$-0.152$, $-0.074$] & $-0.045$ / $-0.021$ / $-0.015$ & $-0.027$ [$-0.104$, $+0.057$] & $-0.023$ / $-0.057$\sig / $-0.043$ & $-0.041$\sig [$-0.071$, $-0.012$] \\
{\mono}@5 $-$ {\mono}@50 & $-0.057$\sig / $-0.058$\sig / $-0.087$\sig & $-0.067$\sig [$-0.091$, $-0.043$] & $-0.070$ / $-0.093$\sig / $-0.080$\sig & $-0.081$\sig [$-0.126$, $-0.033$] & $-0.004$ / $-0.013$ / $-0.002$ & $-0.006$ [$-0.027$, $+0.014$] \\
{\mono}@3 $-$ {\mono}@50 & $-0.080$\sig / $-0.079$\sig / $-0.116$\sig & $-0.092$\sig [$-0.121$, $-0.063$] & $-0.118$\sig / $-0.193$\sig / $-0.216$\sig & $-0.176$\sig [$-0.233$, $-0.110$] & $+0.063$\sig / $+0.002$ / $-0.005$ & $+0.020$ [$-0.006$, $+0.045$] \\
Standalone \M{0}@50 $-$ {\mono}@50 & $+0.068$\sig / $+0.040$ / $+0.010$ & $+0.039$\sig [$+0.009$, $+0.072$] & $+0.162$\sig / $+0.192$\sig / $+0.190$\sig & $+0.182$\sig [$+0.115$, $+0.250$] & $-0.002$ / $-0.034$ / $-0.003$ & $-0.013$ [$-0.038$, $+0.011$] \\
Standalone \M{0}@5 $-$ {\mono}@50 & $-0.081$\sig / $-0.108$\sig / $-0.107$\sig & $-0.099$\sig [$-0.132$, $-0.064$] & $+0.018$ / $+0.104$ / $+0.116$ & $+0.079$\sig [$+0.000$, $+0.154$] & $-0.025$ / $-0.032$ / $-0.033$ & $-0.030$\sig [$-0.055$, $-0.007$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{Step count within a model}} \\
\M{1}@5 $-$ \M{1}@50 & $-0.112$\sig / $-0.134$\sig / $-0.058$\sig & $-0.101$\sig [$-0.127$, $-0.077$] & $-0.101$\sig / $-0.065$ / $-0.096$\sig & $-0.087$\sig [$-0.133$, $-0.037$] & $-0.014$ / $-0.016$ / $-0.015$ & $-0.015$ [$-0.038$, $+0.007$] \\
\M{1}@3 $-$ \M{1}@5 & $-0.016$ / $-0.005$ / $-0.036$\sig & $-0.019$\sig [$-0.040$, $-0.001$] & $-0.003$ / $-0.089$\sig / $-0.010$ & $-0.034$ [$-0.079$, $+0.018$] & $+0.013$ / $-0.032$ / $-0.021$ & $-0.013$ [$-0.034$, $+0.008$] \\
\M{1}@2 $-$ \M{1}@5 & $+0.002$ / $-0.014$ / $-0.039$ & $-0.017$ [$-0.044$, $+0.011$] & $+0.126$\sig / $-0.040$ / $+0.101$\sig & $+0.062$ [$-0.004$, $+0.135$] & $-0.012$ / $-0.014$ / $-0.016$ & $-0.014$ [$-0.041$, $+0.013$] \\
\M{4}@5 $-$ \M{4}@50 & $-0.106$\sig / $-0.081$\sig / $-0.093$\sig & $-0.093$\sig [$-0.119$, $-0.071$] & $-0.094$\sig / $-0.083$ / $-0.001$ & $-0.059$\sig [$-0.107$, $-0.009$] & $-0.027$ / $-0.005$ / $-0.038$\sig & $-0.023$\sig [$-0.043$, $-0.002$] \\
\M{4}@2 $-$ \M{4}@5 & $-0.022$ / $-0.043$\sig / $-0.019$ & $-0.028$ [$-0.058$, $+0.001$] & $+0.049$ / $-0.046$ / $-0.049$ & $-0.015$ [$-0.085$, $+0.057$] & $-0.003$ / $-0.003$ / $-0.013$ & $-0.006$ [$-0.034$, $+0.021$] \\
\M{4}@2 $-$ \M{4}@50 & $-0.128$\sig / $-0.124$\sig / $-0.112$\sig & $-0.121$\sig [$-0.158$, $-0.087$] & $-0.044$ / $-0.129$\sig / $-0.050$ & $-0.074$\sig [$-0.150$, $-0.006$] & $-0.029$ / $-0.008$ / $-0.051$\sig & $-0.030$\sig [$-0.059$, $-0.002$] \\
Standalone \M{1}@5 $-$ Standalone \M{1}@50 & $-0.071$\sig / $-0.091$\sig / $-0.103$\sig & $-0.089$\sig [$-0.114$, $-0.065$] & $-0.132$\sig / $-0.095$\sig / $-0.105$\sig & $-0.111$\sig [$-0.156$, $-0.063$] & $-0.020$ / $-0.021$ / $-0.042$\sig & $-0.028$\sig [$-0.050$, $-0.008$] \\
Standalone \M{0}@5 $-$ Standalone \M{0}@50 & $-0.149$\sig / $-0.148$\sig / $-0.117$\sig & $-0.138$\sig [$-0.169$, $-0.110$] & $-0.144$\sig / $-0.088$ / $-0.075$ & $-0.102$\sig [$-0.160$, $-0.049$] & $-0.024$ / $+0.002$ / $-0.030$ & $-0.017$ [$-0.038$, $+0.006$] \\
{\mono}@3 $-$ {\mono}@5 & $-0.023$ / $-0.021$ / $-0.029$ & $-0.024$\sig [$-0.045$, $-0.004$] & $-0.048$ / $-0.100$\sig / $-0.136$\sig & $-0.094$\sig [$-0.135$, $-0.050$] & $+0.067$\sig / $+0.014$ / $-0.003$ & $+0.026$\sig [$+0.007$, $+0.046$] \\
{\mono}@2 $-$ {\mono}@5 & $-0.031$ / $-0.041$\sig / $-0.020$ & $-0.031$\sig [$-0.063$, $-0.003$] & $-0.072$ / $-0.046$ / $-0.027$ & $-0.048$ [$-0.108$, $+0.022$] & $+0.091$\sig / $+0.043$\sig / $+0.054$\sig & $+0.063$\sig [$+0.031$, $+0.092$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{Second-order solvers at matched compute ($S{=}3$, 4 evaluations per frame)}} \\
\M{1}@3, Heun $-$ \M{1}@5 & $+0.146$\sig / $+0.155$\sig / $+0.122$\sig & $+0.141$\sig [$+0.111$, $+0.173$] & $+0.120$\sig / $-0.001$ / $+0.033$ & $+0.051$\sig [$+0.003$, $+0.101$] & $-0.007$ / $-0.001$ / $+0.007$ & $0.000$ [$-0.024$, $+0.022$] \\
\M{1}@3, midpoint $-$ \M{1}@5 & $+0.108$\sig / $+0.121$\sig / $+0.072$\sig & $+0.101$\sig [$+0.076$, $+0.126$] & $+0.105$\sig / $+0.019$ / $+0.009$ & $+0.044$\sig [$+0.001$, $+0.090$] & $+0.015$ / $+0.028$ / $+0.021$ & $+0.021$ [$-0.002$, $+0.045$] \\
{\mono}@3, Heun $-$ {\mono}@5 & $+0.088$\sig / $+0.078$\sig / $+0.106$\sig & $+0.091$\sig [$+0.063$, $+0.118$] & $+0.049$ / $+0.081$\sig / $+0.040$ & $+0.057$\sig [$+0.014$, $+0.104$] & $+0.038$\sig / $+0.026$ / $+0.007$ & $+0.024$\sig [$+0.003$, $+0.045$] \\
{\mono}@3, midpoint $-$ {\mono}@5 & $+0.092$\sig / $+0.070$\sig / $+0.081$\sig & $+0.081$\sig [$+0.057$, $+0.105$] & $+0.002$ / $-0.016$ / $-0.002$ & $-0.005$ [$-0.050$, $+0.036$] & $+0.022$ / $-0.007$ / $+0.009$ & $+0.008$ [$-0.013$, $+0.027$] \\
\M{1}@3, Heun $-$ \M{1}@50 & $+0.034$ / $+0.020$ / $+0.065$\sig & $+0.040$\sig [$+0.013$, $+0.069$] & $+0.019$ / $-0.066$ / $-0.063$ & $-0.037$ [$-0.087$, $+0.014$] & $-0.021$ / $-0.018$ / $-0.008$ & $-0.016$ [$-0.038$, $+0.006$] \\
\M{1}@3, midpoint $-$ \M{1}@50 & $-0.004$ / $-0.013$ / $+0.014$ & $-0.001$ [$-0.021$, $+0.021$] & $+0.003$ / $-0.046$ / $-0.087$\sig & $-0.043$ [$-0.084$, $+0.004$] & $+0.001$ / $+0.012$ / $+0.006$ & $+0.006$ [$-0.013$, $+0.024$] \\
{\mono}@3, Heun $-$ {\mono}@50 & $+0.031$ / $+0.020$ / $+0.019$ & $+0.023$ [$-0.004$, $+0.050$] & $-0.021$ / $-0.012$ / $-0.040$ & $-0.025$ [$-0.076$, $+0.032$] & $+0.034$ / $+0.013$ / $+0.006$ & $+0.018$ [$-0.004$, $+0.040$] \\
{\mono}@3, midpoint $-$ {\mono}@50 & $+0.035$\sig / $+0.013$ / $-0.006$ & $+0.014$ [$-0.006$, $+0.036$] & $-0.068$ / $-0.109$\sig / $-0.082$\sig & $-0.087$\sig [$-0.128$, $-0.040$] & $+0.018$ / $-0.020$ / $+0.007$ & $+0.002$ [$-0.015$, $+0.019$] \\
\M{1}@3, midpoint $-$ \M{1}@3, Heun & $-0.038$ / $-0.033$ / $-0.051$\sig & $-0.041$\sig [$-0.068$, $-0.014$] & $-0.016$ / $+0.020$ / $-0.024$ & $-0.007$ [$-0.051$, $+0.038$] & $+0.022$ / $+0.030$ / $+0.013$ & $+0.022$\sig [$+0.004$, $+0.042$] \\
{\mono}@3, midpoint $-$ {\mono}@3, Heun & $+0.004$ / $-0.008$ / $-0.025$ & $-0.009$ [$-0.034$, $+0.015$] & $-0.047$ / $-0.097$\sig / $-0.043$ & $-0.062$\sig [$-0.106$, $-0.020$] & $-0.016$ / $-0.033$ / $+0.001$ & $-0.016$ [$-0.036$, $+0.004$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{Uniform-grid second-order solvers ($\alpha{=}1$, 4 evaluations per frame)}} \\
\M{1} unif.\ Heun $-$ \M{1}@5 & $+0.074$\sig / $+0.087$\sig / $+0.050$\sig & $+0.071$\sig [$+0.043$, $+0.102$] & $+0.070$ / $-0.053$ / $-0.005$ & $+0.004$ [$-0.061$, $+0.072$] & $+0.010$ / $+0.005$ / $+0.025$ & $+0.014$ [$-0.010$, $+0.039$] \\
\M{1} unif.\ midpoint $-$ \M{1}@5 & $+0.101$\sig / $+0.146$\sig / $+0.078$\sig & $+0.108$\sig [$+0.082$, $+0.136$] & $+0.074$ / $-0.042$ / $-0.044$ & $-0.004$ [$-0.060$, $+0.051$] & $+0.011$ / $+0.000$ / $+0.039$ & $+0.017$ [$-0.008$, $+0.042$] \\
{\mono} unif.\ Heun $-$ {\mono}@5 & $+0.050$\sig / $+0.051$\sig / $+0.072$\sig & $+0.058$\sig [$+0.029$, $+0.086$] & $-0.044$ / $-0.016$ / $-0.067$ & $-0.042$ [$-0.093$, $+0.015$] & $+0.001$ / $+0.012$ / $+0.012$ & $+0.008$ [$-0.016$, $+0.033$] \\
{\mono} unif.\ midpoint $-$ {\mono}@5 & $+0.072$\sig / $+0.091$\sig / $+0.108$\sig & $+0.090$\sig [$+0.062$, $+0.121$] & $+0.017$ / $-0.040$ / $-0.062$ & $-0.028$ [$-0.079$, $+0.023$] & $+0.033$ / $+0.000$ / $+0.015$ & $+0.016$ [$-0.005$, $+0.038$] \\
\M{1} unif.\ Heun $-$ \M{1}@3, Heun & $-0.072$\sig / $-0.067$\sig / $-0.072$\sig & $-0.071$\sig [$-0.101$, $-0.040$] & $-0.050$ / $-0.052$ / $-0.038$ & $-0.047$ [$-0.100$, $+0.008$] & $+0.018$ / $+0.007$ / $+0.018$ & $+0.014$ [$-0.008$, $+0.035$] \\
\M{1} unif.\ midpoint $-$ \M{1}@3, midpoint & $-0.007$ / $+0.024$ / $+0.006$ & $+0.008$ [$-0.019$, $+0.033$] & $-0.031$ / $-0.061$ / $-0.053$ & $-0.048$ [$-0.097$, $+0.007$] & $-0.003$ / $-0.028$ / $+0.018$ & $-0.004$ [$-0.025$, $+0.017$] \\
{\mono} unif.\ Heun $-$ {\mono}@3, Heun & $-0.039$ / $-0.027$ / $-0.034$ & $-0.033$\sig [$-0.062$, $-0.004$] & $-0.092$\sig / $-0.096$\sig / $-0.108$\sig & $-0.099$\sig [$-0.151$, $-0.045$] & $-0.037$ / $-0.014$ / $+0.005$ & $-0.015$ [$-0.037$, $+0.007$] \\
{\mono} unif.\ midpoint $-$ {\mono}@3, midpoint & $-0.020$ / $+0.021$ / $+0.026$ & $+0.009$ [$-0.016$, $+0.041$] & $+0.015$ / $-0.024$ / $-0.060$ & $-0.023$ [$-0.074$, $+0.031$] & $+0.011$ / $+0.008$ / $+0.006$ & $+0.008$ [$-0.013$, $+0.030$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{Symmetric multi-draw score averaging ($3{,}840\text{--}11{,}520$ evaluations per decision)}} \\
\M{1}@3 (2 draws) $-$ {\mono}@3 (2 draws) & $-0.024$ / $-0.034$ / $+0.014$ & $-0.015$ [$-0.043$, $+0.012$] & $+0.001$ / $+0.108$\sig / $-0.001$ & $+0.036$ [$-0.027$, $+0.097$] & $-0.055$\sig / $-0.073$\sig / $-0.015$ & $-0.048$\sig [$-0.077$, $-0.021$] \\
\M{4}@3 (2 draws) $-$ {\mono}@3 (2 draws) & $-0.008$ / $-0.029$ / $-0.014$ & $-0.017$ [$-0.044$, $+0.008$] & $+0.064$ / $+0.066$ / $+0.028$ & $+0.053$ [$-0.012$, $+0.114$] & $-0.054$\sig / $-0.080$\sig / $-0.038$ & $-0.057$\sig [$-0.083$, $-0.030$] \\
\M{1}@3 (2 draws) $-$ \M{4}@3 (2 draws) & $-0.015$ / $-0.005$ / $+0.027$ & $+0.002$ [$-0.015$, $+0.021$] & $-0.063$\sig / $+0.042$ / $-0.029$ & $-0.017$ [$-0.053$, $+0.026$] & $-0.001$ / $+0.007$ / $+0.023$ & $+0.010$ [$-0.010$, $+0.029$] \\
\M{1}@2 (4 draws) $-$ {\mono}@2 (4 draws) & $+0.001$ / $-0.006$ / $-0.013$ & $-0.006$ [$-0.039$, $+0.027$] & $+0.112$\sig / $+0.093$ / $+0.076$ & $+0.094$\sig [$+0.023$, $+0.171$] & $-0.082$\sig / $-0.114$\sig / $-0.071$\sig & $-0.089$\sig [$-0.120$, $-0.058$] \\
\M{1}@3 (2 draws) $-$ \M{1}@5 & $-0.024$ / $-0.016$ / $-0.039$\sig & $-0.026$\sig [$-0.050$, $-0.004$] & $-0.064$ / $-0.167$\sig / $-0.134$\sig & $-0.122$\sig [$-0.171$, $-0.070$] & $+0.005$ / $-0.034$ / $+0.008$ & $-0.007$ [$-0.030$, $+0.016$] \\
\M{1}@3 (2 draws) $-$ \M{1}@3 & $-0.007$ / $-0.011$ / $-0.002$ & $-0.007$ [$-0.021$, $+0.009$] & $-0.062$\sig / $-0.077$\sig / $-0.124$\sig & $-0.088$\sig [$-0.121$, $-0.054$] & $-0.008$ / $-0.002$ / $+0.029$ & $+0.006$ [$-0.012$, $+0.024$] \\
\M{1}@3 (2 draws) $-$ \M{1}@2 (4 draws) & $-0.027$ / $-0.017$ / $-0.006$ & $-0.016$ [$-0.038$, $+0.004$] & $-0.157$\sig / $-0.072$ / $-0.159$\sig & $-0.130$\sig [$-0.192$, $-0.066$] & $+0.005$ / $-0.004$ / $+0.014$ & $+0.005$ [$-0.017$, $+0.028$] \\
{\mono}@3 (2 draws) $-$ {\mono}@5 & $-0.035$ / $-0.036$ / $-0.050$\sig & $-0.040$\sig [$-0.063$, $-0.018$] & $-0.166$\sig / $-0.162$\sig / $-0.168$\sig & $-0.165$\sig [$-0.213$, $-0.117$] & $+0.053$\sig / $+0.008$ / $-0.003$ & $+0.020$ [$-0.004$, $+0.043$] \\
{\mono}@3 (2 draws) $-$ {\mono}@3 & $-0.012$ / $-0.015$ / $-0.022$ & $-0.016$\sig [$-0.030$, $-0.002$] & $-0.118$\sig / $-0.062$\sig / $-0.032$ & $-0.071$\sig [$-0.106$, $-0.037$] & $-0.014$ / $-0.006$ / $0.000$ & $-0.007$ [$-0.025$, $+0.010$] \\
{\mono}@3 (2 draws) $-$ {\mono}@50 & $-0.092$\sig / $-0.094$\sig / $-0.137$\sig & $-0.108$\sig [$-0.137$, $-0.077$] & $-0.236$\sig / $-0.255$\sig / $-0.248$\sig & $-0.247$\sig [$-0.309$, $-0.181$] & $+0.049$\sig / $-0.004$ / $-0.004$ & $+0.013$ [$-0.012$, $+0.039$] \\
{\mono}@3 (2 draws) $-$ {\mono}@2 (4 draws) & $-0.003$ / $+0.012$ / $-0.032$ & $-0.008$ [$-0.033$, $+0.017$] & $-0.046$ / $-0.087$ / $-0.082$ & $-0.072$\sig [$-0.130$, $-0.012$] & $-0.022$ / $-0.045$\sig / $-0.042$\sig & $-0.036$\sig [$-0.059$, $-0.013$] \\
{\mono}@2 (4 draws) $-$ {\mono}@5 & $-0.032$ / $-0.048$\sig / $-0.018$ & $-0.033$\sig [$-0.064$, $-0.003$] & $-0.120$\sig / $-0.075$ / $-0.086$ & $-0.094$\sig [$-0.158$, $-0.024$] & $+0.075$\sig / $+0.053$\sig / $+0.040$ & $+0.056$\sig [$+0.026$, $+0.085$] \\
\M{4}@3 (2 draws) $-$ \M{4}@5 & $-0.019$ / $-0.049$\sig / $-0.033$ & $-0.034$\sig [$-0.059$, $-0.007$] & $-0.037$ / $-0.173$\sig / $-0.174$\sig & $-0.128$\sig [$-0.175$, $-0.076$] & $+0.009$ / $-0.030$ / $-0.013$ & $-0.011$ [$-0.035$, $+0.012$] \\
\M{4}@3 (2 draws) $-$ \M{4}@50 & $-0.125$\sig / $-0.130$\sig / $-0.126$\sig & $-0.127$\sig [$-0.162$, $-0.095$] & $-0.130$\sig / $-0.256$\sig / $-0.175$\sig & $-0.187$\sig [$-0.243$, $-0.128$] & $-0.017$ / $-0.035$ / $-0.051$\sig & $-0.034$\sig [$-0.061$, $-0.010$] \\
\M{1}@5 (3 draws) $-$ \M{1}@50 & $-0.124$\sig / $-0.130$\sig / $-0.107$\sig & $-0.120$\sig [$-0.147$, $-0.093$] & $-0.177$\sig / $-0.276$\sig / $-0.279$\sig & $-0.244$\sig [$-0.298$, $-0.185$] & $-0.008$ / $-0.053$\sig / $-0.022$ & $-0.027$\sig [$-0.053$, $-0.004$] \\
\M{1}@3 (2 draws) $-$ \M{1}@5 (3 draws) & $-0.012$ / $-0.020$ / $+0.011$ & $-0.007$ [$-0.029$, $+0.014$] & $+0.011$ / $+0.044$ / $+0.049$ & $+0.035$ [$-0.011$, $+0.079$] & $-0.001$ / $+0.002$ / $+0.014$ & $+0.005$ [$-0.017$, $+0.028$] \\
\midrule
5\,\% margin & \multicolumn{2}{c}{0.068} & \multicolumn{2}{c}{0.142} & \multicolumn{2}{c}{0.052} \\


==> tab/gen/supp_r4_r5_ci_body.tex <==
\multicolumn{4}{@{}l}{\emph{Symmetric two-draw score averaging at three steps ($S{=}3$, $3{,}840$ evaluations, seeds 0--2)}} \\
2 draws \at{1}{3} ($3{,}840$) $-$ 2 draws \monoat{3} ($3{,}840$) & $-0.015$ [$-0.043$, $+0.012$] & $+0.036$ [$-0.027$, $+0.097$] & $-0.048$\sig [$-0.077$, $-0.021$] \\
2 draws \at{4}{3} ($3{,}840$) $-$ 2 draws \monoat{3} ($3{,}840$) & $-0.017$ [$-0.044$, $+0.008$] & $+0.053$ [$-0.012$, $+0.114$] & $-0.057$\sig [$-0.083$, $-0.030$] \\
2 draws \at{1}{3} ($3{,}840$) $-$ 1 draw \at{1}{5} ($3{,}840$) & $-0.026$\sig [$-0.050$, $-0.004$] & $-0.122$\sig [$-0.171$, $-0.070$] & $-0.007$ [$-0.030$, $+0.016$] \\
2 draws \at{1}{3} ($3{,}840$) $-$ 1 draw \at{1}{3} ($1{,}920$) & $-0.007$ [$-0.021$, $+0.009$] & $-0.088$\sig [$-0.121$, $-0.054$] & $+0.006$ [$-0.012$, $+0.024$] \\
2 draws \at{1}{3} ($3{,}840$) $-$ 1 draw \at{1}{50} ($47{,}040$) & $-0.127$\sig [$-0.159$, $-0.096$] & $-0.209$\sig [$-0.268$, $-0.147$] & $-0.022$ [$-0.053$, $+0.005$] \\
2 draws \monoat{3} ($3{,}840$) $-$ 1 draw \monoat{5} ($3{,}840$) & $-0.040$\sig [$-0.063$, $-0.018$] & $-0.165$\sig [$-0.213$, $-0.117$] & $+0.020$ [$-0.004$, $+0.043$] \\
2 draws \monoat{3} ($3{,}840$) $-$ 1 draw \monoat{3} ($1{,}920$) & $-0.016$\sig [$-0.030$, $-0.002$] & $-0.071$\sig [$-0.106$, $-0.037$] & $-0.007$ [$-0.025$, $+0.010$] \\
2 draws \monoat{3} ($3{,}840$) $-$ 1 draw \monoat{50} ($47{,}040$) & $-0.108$\sig [$-0.137$, $-0.077$] & $-0.247$\sig [$-0.309$, $-0.181$] & $+0.013$ [$-0.012$, $+0.039$] \\
2 draws \at{4}{3} ($3{,}840$) $-$ 1 draw \at{4}{5} ($3{,}840$) & $-0.034$\sig [$-0.059$, $-0.007$] & $-0.128$\sig [$-0.175$, $-0.076$] & $-0.011$ [$-0.035$, $+0.012$] \\
2 draws \at{4}{3} ($3{,}840$) $-$ 1 draw \at{4}{50} ($47{,}040$) & $-0.127$\sig [$-0.162$, $-0.095$] & $-0.187$\sig [$-0.243$, $-0.128$] & $-0.034$\sig [$-0.061$, $-0.010$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{Four-draw score averaging at two steps ($S{=}2$, $3{,}840$ evaluations, seeds 0--2)}} \\
4 draws \at{1}{2} ($3{,}840$) $-$ 1 draw \at{1}{5} ($3{,}840$) & $-0.010$ [$-0.038$, $+0.020$] & $+0.008$ [$-0.062$, $+0.084$] & $-0.012$ [$-0.040$, $+0.013$] \\
4 draws \at{1}{2} ($3{,}840$) $-$ 2 draws \at{1}{3} ($3{,}840$) & $+0.016$ [$-0.004$, $+0.038$] & $+0.130$\sig [$+0.066$, $+0.192$] & $-0.005$ [$-0.028$, $+0.017$] \\
4 draws \at{1}{2} ($3{,}840$) $-$ 1 draw \at{1}{2} (mean over 4 draws) & $+0.006$ [$-0.002$, $+0.014$] & $-0.036$\sig [$-0.056$, $-0.015$] & $-0.002$ [$-0.010$, $+0.007$] \\
4 draws \monoat{2} ($3{,}840$) $-$ 1 draw \monoat{5} ($3{,}840$) & $-0.033$\sig [$-0.064$, $-0.003$] & $-0.094$\sig [$-0.158$, $-0.024$] & $+0.056$\sig [$+0.026$, $+0.085$] \\
4 draws \monoat{2} ($3{,}840$) $-$ 2 draws \monoat{3} ($3{,}840$) & $+0.008$ [$-0.017$, $+0.033$] & $+0.072$\sig [$+0.012$, $+0.130$] & $+0.036$\sig [$+0.013$, $+0.059$] \\
4 draws \monoat{2} ($3{,}840$) $-$ 1 draw \monoat{2} (mean over 4 draws) & $-0.001$ [$-0.009$, $+0.007$] & $-0.029$\sig [$-0.048$, $-0.009$] & $-0.003$ [$-0.011$, $+0.005$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{Three-seed multi-draw score averaging at five steps (\at{1}{5}, $M{=}3$, seeds 0--2) and seed-0 \at{1}{50} ($n{=}500$)}} \\
2 draws \at{1}{3} ($3{,}840$) $-$ 2 draws \at{1}{5} ($7{,}680$) & $-0.011$ [$-0.029$, $+0.007$] & $-0.012$ [$-0.049$, $+0.029$] & $+0.003$ [$-0.017$, $+0.020$] \\
2 draws \at{1}{3} ($3{,}840$) $-$ 3 draws \at{1}{5} ($11{,}520$) & $-0.007$ [$-0.029$, $+0.014$] & $+0.035$ [$-0.011$, $+0.079$] & $+0.005$ [$-0.017$, $+0.028$] \\
2 draws \at{1}{5} ($7{,}680$) $-$ 1 draw \at{1}{5} (mean over 3 draws) & $-0.026$\sig [$-0.035$, $-0.017$] & $-0.116$\sig [$-0.139$, $-0.092$] & $-0.003$ [$-0.014$, $+0.008$] \\
3 draws \at{1}{5} ($11{,}520$) $-$ 1 draw \at{1}{5} (mean over 3 draws) & $-0.030$\sig [$-0.045$, $-0.017$] & $-0.162$\sig [$-0.196$, $-0.126$] & $-0.006$ [$-0.021$, $+0.010$] \\
3 draws \at{1}{5} ($11{,}520$) $-$ 1 draw \at{1}{50} ($47{,}040$) & $-0.120$\sig [$-0.147$, $-0.093$] & $-0.244$\sig [$-0.298$, $-0.185$] & $-0.027$\sig [$-0.053$, $-0.004$] \\
Seed 0: 3 draws \at{1}{50} ($141{,}120$) $-$ 1 draw \at{1}{50} (mean over 3 draws) & $-0.038$\sig [$-0.070$, $-0.006$] & $-0.183$\sig [$-0.245$, $-0.113$] & -- \\
Seed 0: 3 draws \at{1}{50} ($141{,}120$) $-$ 2 draws \at{1}{3} ($3{,}840$) & $+0.105$\sig [$+0.058$, $+0.151$] & $+0.024$ [$-0.071$, $+0.114$] & -- \\
Seed 0: 3 draws \at{1}{50} ($141{,}120$) $-$ 1 draw \at{1}{5} (mean over 3 draws) & $+0.071$\sig [$+0.034$, $+0.109$] & $-0.092$\sig [$-0.165$, $-0.022$] & -- \\
Seed 0: 3 draws \at{1}{50} ($141{,}120$) $-$ 3 draws \at{1}{5} ($11{,}520$) & $+0.094$\sig [$+0.051$, $+0.134$] & $+0.035$ [$-0.044$, $+0.111$] & -- \\
\midrule
\multicolumn{4}{@{}l}{\emph{Three-draw second-order solvers vs.\ three-draw five-step Euler (seed 0, $n{=}100$ nested shard 0/5)}} \\
Seed 0 ($n{=}100$): 3 draws \M{1} Heun@3 $-$ 3 draws \at{1}{5} ($11{,}520$) & $+0.157$\sig [$+0.064$, $+0.248$] & $+0.258$\sig [$+0.097$, $+0.430$] & $-0.034$ [$-0.117$, $+0.046$] \\
Seed 0 ($n{=}100$): 3 draws \M{1} midpoint@3 $-$ 3 draws \at{1}{5} ($11{,}520$) & $+0.112$\sig [$+0.030$, $+0.193$] & $+0.056$ [$-0.080$, $+0.199$] & $-0.008$ [$-0.087$, $+0.071$] \\


==> tab/gen/supp_sdpa_shard_body.tex <==
\mono & 50 / 49 & 80.9 (1.0$\times$) & -- & -- & 52.1 (1.0$\times$) & 51.9$^{\dagger}$ (1.0$\times$) & 187.4 (1.0$\times$) & 2.805 / 2.789 & $+0.559^{\dagger}$ \ci{$-0.016$, $+1.102$} \\
\paper \M{4} & 50 / 49 & 80.8 (1.0$\times$) & -- & -- & 53.2 (1.0$\times$) & 53.2$^{\dagger}$ (1.0$\times$) & 187.7 (1.0$\times$) & 2.679 / 2.698 & $+0.320^{\dagger}$ \ci{$-0.122$, $+0.799$} \\
\paper \M{1} & 50 / 49 & 68.8 (1.2$\times$) & -- & -- & 39.8 (1.3$\times$) & 39.8$^{\dagger}$ (1.3$\times$) & 176.1 (1.1$\times$) & 2.947 / 2.941 & $+0.176^{\dagger}$ \ci{$-0.283$, $+0.599$} \\
\midrule
\mono & 5 / 4 & 6.92 (11.7$\times$) & 6.70 & 4.64 & 4.40 (11.8$\times$) & 4.30 (12.1$\times$) & 15.7 (11.9$\times$) & 2.873 / 2.886 & $-0.158$ \ci{$-0.430$, $+0.104$} \\
\paper \M{4} & 5 / 4 & 6.97 (11.6$\times$) & 6.73 & 4.69 & 4.44 (11.7$\times$) & 4.37 (11.9$\times$) & 15.7 (11.9$\times$) & 2.948 / 2.948 & $-0.176$ \ci{$-0.415$, $+0.080$} \\
\paper \M{1} & 5 / 4 & 5.91 (13.7$\times$) & 5.65 & 3.60 & 3.35 (15.6$\times$) & 3.27 (15.9$\times$) & 14.8 (12.7$\times$) & 2.724 / 2.741 & $-0.069$ \ci{$-0.335$, $+0.172$} \\
\midrule
\mono (2 draws) & 3 / 2 & 7.23 (11.2$\times$) & 6.74 & 4.95 & 4.48 (11.6$\times$) & 4.26 (12.2$\times$) & 16.0 (11.7$\times$) & 2.776 / 2.736 & $-0.017$ \ci{$-0.215$, $+0.188$} \\
\paper \M{4} (2 draws) & 3 / 2 & 7.27 (11.1$\times$) & 6.77 & 5.02 & 4.49 (11.6$\times$) & 4.35 (11.9$\times$) & 16.1 (11.6$\times$) & 2.789 / 2.789 & $+0.143$ \ci{$-0.068$, $+0.359$} \\
\paper \M{1} (2 draws) & 3 / 2 & 6.17 (13.1$\times$) & 5.66 & 3.90 & 3.39 (15.4$\times$) & 3.24 (16.0$\times$) & 15.1 (12.4$\times$) & 2.686 / 2.686 & $+0.155$ \ci{$-0.040$, $+0.342$} \\
\midrule
\mono & 3 / 2 & 3.64 (22.2$\times$) & 3.42 & 2.48 & 2.26 (23.0$\times$) & 2.15 (24.1$\times$) & 8.01 (23.4$\times$) & 2.931 / 2.917 & $-0.156$ \ci{$-0.364$, $+0.042$} \\
\paper \M{4} & 3 / 2 & 3.66 (22.1$\times$) & 3.42 & 2.51 & 2.26 (23.1$\times$) & 2.19 (23.7$\times$) & 8.08 (23.2$\times$) & 2.940 / 2.986 & $+0.022$ \ci{$-0.246$, $+0.264$} \\
\paper \M{1} & 3 / 2 & 3.13 (25.8$\times$) & 2.88 & 1.98 & 1.72 (30.3$\times$) & 1.64 (31.6$\times$) & 7.57 (24.8$\times$) & 2.789 / 2.789 & $+0.051$ \ci{$-0.162$, $+0.276$} \\
\midrule
\mono & 2 / 1 & 1.98 (40.8$\times$) & 1.78 & 1.59 & 1.19 (43.8$\times$) & 1.08 (47.9$\times$) & 4.19 (44.7$\times$) & 2.894 / 2.919 & $-0.202$ \ci{$-0.409$, $+0.001$} \\
\paper \M{4} & 2 / 1 & 2.00 (40.4$\times$) & 1.76 & 1.60 & 1.17 (44.4$\times$) & 1.10 (47.1$\times$) & 4.22 (44.4$\times$) & 2.785 / 2.797 & $+0.091$ \ci{$-0.106$, $+0.293$} \\
\paper \M{1} & 2 / 1 & 1.78 (45.4$\times$) & 1.49 & 1.60 & 0.91 (57.4$\times$) & 0.83 (62.6$\times$) & 3.96 (47.3$\times$) & 2.660 / 2.663 & $+0.062$ \ci{$-0.173$, $+0.260$} \\


==> tab/gen/supp_seeds_body.tex <==
All-\M{1} & 50 & 1.37 / 1.39 / 1.34 ($1.37\pm0.02$) & 2.78 / 2.89 / 2.84 ($2.84\pm0.06$) & 1.01 / 1.02 / 1.04 ($1.03\pm0.01$) \\
 & 20 & 1.34 / 1.36 / 1.33 ($1.35\pm0.02$) & 2.79 / 2.87 / 2.84 ($2.83\pm0.04$) & 1.02 / 1.03 / 1.07 ($1.04\pm0.03$) \\
 & 10 & 1.32 / 1.32 / 1.30 ($1.31\pm0.01$) & 2.74 / 2.83 / 2.76 ($2.78\pm0.05$) & 0.99 / 1.01 / 1.05 ($1.02\pm0.03$) \\
 & 5 & 1.26 / 1.26 / 1.28 ($1.27\pm0.02$) & 2.68 / 2.83 / 2.74 ($2.75\pm0.08$) & 1.00 / 1.00 / 1.03 ($1.01\pm0.01$) \\
 & 5, 2 draws & 1.25 / 1.26 / 1.24 ($1.25\pm0.01$) & 2.63 / 2.68 / 2.60 ($2.64\pm0.04$) & 1.01 / 0.97 / 1.03 ($1.00\pm0.03$) \\
 & 5, 3 draws & 1.25 / 1.26 / 1.24 ($1.25\pm0.01$) & 2.60 / 2.62 / 2.56 ($2.59\pm0.03$) & 1.01 / 0.97 / 1.02 ($1.00\pm0.03$) \\
 & 4 & 1.27 / 1.26 / 1.25 ($1.26\pm0.01$) & 2.67 / 2.79 / 2.68 ($2.71\pm0.07$) & 1.00 / 1.00 / 1.02 ($1.01\pm0.01$) \\
 & 3 & 1.24 / 1.25 / 1.25 ($1.25\pm0.00$) & 2.67 / 2.74 / 2.73 ($2.71\pm0.04$) & 1.01 / 0.97 / 1.01 ($1.00\pm0.02$) \\
 & 3, 2 draws & 1.24 / 1.24 / 1.25 ($1.24\pm0.01$) & 2.61 / 2.66 / 2.61 ($2.63\pm0.03$) & 1.01 / 0.97 / 1.03 ($1.00\pm0.03$) \\
 & 3, Heun & 1.41 / 1.41 / 1.41 ($1.41\pm0.00$) & 2.80 / 2.83 / 2.77 ($2.80\pm0.03$) & 0.99 / 1.00 / 1.03 ($1.01\pm0.02$) \\
 & 3, midpoint & 1.37 / 1.38 / 1.36 ($1.37\pm0.01$) & 2.78 / 2.85 / 2.75 ($2.79\pm0.05$) & 1.01 / 1.03 / 1.05 ($1.03\pm0.02$) \\
 & unif.\ Euler ($\alpha{=}1$) & 1.27 / 1.29 / 1.29 ($1.28\pm0.01$) & 2.70 / 2.78 / 2.72 ($2.73\pm0.04$) & 0.99 / 0.99 / 1.02 ($1.00\pm0.02$) \\
 & unif.\ Heun ($\alpha{=}1$) & 1.33 / 1.34 / 1.33 ($1.34\pm0.01$) & 2.75 / 2.78 / 2.74 ($2.75\pm0.02$) & 1.01 / 1.01 / 1.05 ($1.02\pm0.02$) \\
 & unif.\ midpoint ($\alpha{=}1$) & 1.36 / 1.40 / 1.36 ($1.37\pm0.02$) & 2.75 / 2.79 / 2.70 ($2.74\pm0.05$) & 1.01 / 1.00 / 1.07 ($1.03\pm0.03$) \\
 & 2 & 1.26 / 1.24 / 1.25 ($1.25\pm0.01$) & 2.80 / 2.79 / 2.84 ($2.81\pm0.03$) & 0.99 / 0.99 / 1.01 ($1.00\pm0.01$) \\
 & 2, 4 draws & 1.26 / 1.26 / 1.25 ($1.26\pm0.01$) & 2.77 / 2.74 / 2.77 ($2.76\pm0.02$) & 1.00 / 0.97 / 1.02 ($1.00\pm0.02$) \\
\midrule
All-\M{4} & 50 & 1.38 / 1.37 / 1.34 ($1.36\pm0.02$) & 2.81 / 2.88 / 2.81 ($2.83\pm0.04$) & 1.02 / 1.00 / 1.06 ($1.03\pm0.03$) \\
 & 5 & 1.27 / 1.29 / 1.25 ($1.27\pm0.02$) & 2.71 / 2.79 / 2.81 ($2.77\pm0.05$) & 1.00 / 0.99 / 1.02 ($1.01\pm0.02$) \\
 & 3 & 1.25 / 1.25 / 1.25 ($1.25\pm0.00$) & 2.69 / 2.76 / 2.77 ($2.74\pm0.04$) & 1.01 / 0.99 / 1.03 ($1.01\pm0.02$) \\
 & 3, 2 draws & 1.25 / 1.24 / 1.22 ($1.24\pm0.02$) & 2.68 / 2.62 / 2.63 ($2.64\pm0.03$) & 1.01 / 0.96 / 1.01 ($0.99\pm0.03$) \\
 & 2 & 1.25 / 1.25 / 1.23 ($1.24\pm0.01$) & 2.76 / 2.75 / 2.76 ($2.76\pm0.01$) & 0.99 / 0.99 / 1.01 ($1.00\pm0.01$) \\
\midrule
\mono & 50 & 1.35 / 1.37 / 1.37 ($1.36\pm0.01$) & 2.85 / 2.81 / 2.86 ($2.84\pm0.02$) & 1.01 / 1.05 / 1.05 ($1.04\pm0.02$) \\
 & 20 & 1.35 / 1.34 / 1.36 ($1.35\pm0.01$) & 2.85 / 2.78 / 2.82 ($2.82\pm0.04$) & 1.03 / 1.05 / 1.07 ($1.05\pm0.02$) \\
 & 10 & 1.32 / 1.35 / 1.31 ($1.33\pm0.02$) & 2.80 / 2.72 / 2.80 ($2.77\pm0.05$) & 1.00 / 1.04 / 1.05 ($1.03\pm0.03$) \\
 & 5 & 1.29 / 1.31 / 1.28 ($1.30\pm0.01$) & 2.78 / 2.72 / 2.78 ($2.76\pm0.03$) & 1.01 / 1.03 / 1.05 ($1.03\pm0.02$) \\
 & 4 & 1.29 / 1.29 / 1.28 ($1.28\pm0.01$) & 2.72 / 2.66 / 2.72 ($2.70\pm0.04$) & 1.04 / 1.01 / 1.05 ($1.03\pm0.02$) \\
 & 3 & 1.27 / 1.29 / 1.25 ($1.27\pm0.02$) & 2.73 / 2.62 / 2.64 ($2.66\pm0.06$) & 1.07 / 1.05 / 1.05 ($1.06\pm0.01$) \\
 & 3, 2 draws & 1.26 / 1.27 / 1.23 ($1.25\pm0.02$) & 2.61 / 2.55 / 2.61 ($2.59\pm0.03$) & 1.06 / 1.04 / 1.05 ($1.05\pm0.01$) \\
 & 3, Heun & 1.38 / 1.39 / 1.39 ($1.39\pm0.00$) & 2.83 / 2.80 / 2.82 ($2.81\pm0.01$) & 1.05 / 1.06 / 1.06 ($1.06\pm0.01$) \\
 & 3, midpoint & 1.39 / 1.38 / 1.36 ($1.38\pm0.01$) & 2.78 / 2.70 / 2.77 ($2.75\pm0.04$) & 1.03 / 1.03 / 1.06 ($1.04\pm0.02$) \\
 & unif.\ Euler ($\alpha{=}1$) & 1.30 / 1.32 / 1.31 ($1.31\pm0.01$) & 2.75 / 2.64 / 2.67 ($2.69\pm0.06$) & 1.01 / 1.04 / 1.07 ($1.04\pm0.03$) \\
 & unif.\ Heun ($\alpha{=}1$) & 1.34 / 1.36 / 1.36 ($1.35\pm0.01$) & 2.73 / 2.70 / 2.71 ($2.71\pm0.02$) & 1.01 / 1.05 / 1.06 ($1.04\pm0.03$) \\
 & unif.\ midpoint ($\alpha{=}1$) & 1.37 / 1.40 / 1.39 ($1.39\pm0.02$) & 2.79 / 2.68 / 2.71 ($2.73\pm0.06$) & 1.04 / 1.03 / 1.07 ($1.05\pm0.02$) \\
 & 2 & 1.26 / 1.27 / 1.26 ($1.26\pm0.00$) & 2.71 / 2.67 / 2.75 ($2.71\pm0.04$) & 1.10 / 1.08 / 1.11 ($1.09\pm0.02$) \\
 & 2, 4 draws & 1.26 / 1.26 / 1.26 ($1.26\pm0.00$) & 2.66 / 2.64 / 2.69 ($2.66\pm0.02$) & 1.08 / 1.09 / 1.09 ($1.09\pm0.00$) \\
\midrule
Standalone \M{1} & 50 & 1.36 / 1.38 / 1.37 ($1.37\pm0.01$) & 2.83 / 2.82 / 2.83 ($2.83\pm0.00$) & 1.00 / 1.01 / 1.05 ($1.02\pm0.02$) \\
 & 5 & 1.28 / 1.29 / 1.27 ($1.28\pm0.01$) & 2.69 / 2.73 / 2.73 ($2.72\pm0.02$) & 0.98 / 0.99 / 1.00 ($0.99\pm0.01$) \\
\midrule
Standalone \M{0} & 50 & 1.42 / 1.41 / 1.38 ($1.40\pm0.02$) & 3.01 / 3.00 / 3.05 ($3.02\pm0.02$) & 1.01 / 1.01 / 1.05 ($1.02\pm0.02$) \\
 & 5 & 1.27 / 1.26 / 1.26 ($1.26\pm0.01$) & 2.87 / 2.91 / 2.97 ($2.92\pm0.05$) & 0.99 / 1.01 / 1.02 ($1.01\pm0.02$) \\
 & 3 & 1.27 / 1.26 / 1.31 ($1.28\pm0.03$) & 2.87 / 2.92 / 2.94 ($2.91\pm0.03$) & 0.99 / 1.02 / 1.00 ($1.01\pm0.01$) \\
 & 2 & 1.27 / 1.29 / 1.29 ($1.29\pm0.01$) & 2.91 / 2.93 / 2.92 ($2.92\pm0.01$) & 1.02 / 1.03 / 1.00 ($1.01\pm0.02$) \\
\midrule
\mono, naive \M{1} slice & 5 & 1.73 / -- / -- (1.73) & 4.86 / -- / -- (4.86) & 1.09 / -- / -- (1.09) \\


==> tab/gen/supp_t13_body.tex <==
\multicolumn{7}{@{}l}{\emph{(a) Two-round iterative \cem (2\,s / 8-step horizon; round 0 = 1-round plan inside the same job)}} \\
\paper \M{1} & \recon & 1.350 / 1.318 & 1.268 / 1.226 & $-0.101$\sig [$-0.153$, $-0.047$] & $-0.107$\sig [$-0.188$, $-0.037$] & $-0.042$\sig [$-0.062$, $-0.021$] / $-0.033$ [$-0.093$, $+0.028$] \\
\paper \M{1} & \sacson & 2.792 / 2.693 & 2.754 / 2.584 & $-0.096$ [$-0.213$, $+0.023$] & $-0.171$\sig [$-0.309$, $-0.030$] & $-0.170$\sig [$-0.239$, $-0.106$] / $-0.099$ [$-0.261$, $+0.053$] \\
\mono & \recon & 1.416 / 1.394 & 1.290 / 1.265 & $-0.110$\sig [$-0.162$, $-0.063$] & $-0.125$\sig [$-0.199$, $-0.059$] & $-0.024$\sig [$-0.045$, $-0.004$] / $-0.022$ [$-0.077$, $+0.031$] \\
\mono & \sacson & 2.738 / 2.580 & 2.753 / 2.599 & $-0.048$ [$-0.147$, $+0.060$] & $+0.017$ [$-0.104$, $+0.140$] & $-0.153$\sig [$-0.219$, $-0.091$] / $-0.158$ [$-0.325$, $+0.002$] \\
\midrule
\multicolumn{7}{@{}l}{\emph{(b) Longer planning horizon: 4\,s / 16 autoregressive steps (1-round \cem; \ate / \rpe and paired $S{=}5 - S{=}50$ on $n{=}100$)}} \\
\paper \M{1} & \recon & 3.347 / 0.537 & 3.234 / 0.524 & $+0.020$ [$-0.101$, $+0.143$] & $+0.015$\sig [$+0.004$, $+0.027$] & -- \\
\paper \M{1} & \sacson & 5.413 / 0.748 & 5.339 / 0.749 & $+0.042$ [$-0.152$, $+0.237$] & $+0.003$ [$-0.018$, $+0.024$] & -- \\
\mono & \recon & 3.366 / 0.538 & 3.210 / 0.519 & $+0.009$ [$-0.120$, $+0.137$] & $+0.011$\sig [$+0.001$, $+0.021$] & -- \\
\mono & \sacson & 5.441 / 0.748 & 5.343 / 0.744 & $+0.040$ [$-0.144$, $+0.231$] & $+0.003$ [$-0.013$, $+0.019$] & -- \\


==> tab/gen/supp_t2_reg_gen_body.tex <==
\recon & DINO-Reg, 25 epochs & 0.4997 & 0.5815 & 0.4809 & 0.5584 & 167.54 & 217.73 \\
 & DINO-Reg, 47 epochs & 0.4669 & 0.5565 & 0.4482 & 0.5218 & 118.72 & 154.48 \\
 & DINO-Reg, 50 epochs & 0.4644 & 0.5542 & 0.4462 & 0.5195 & 115.51 & 149.71 \\
 & \paper \M{1}, $S{=}50$ & 0.3846 & 0.4602 & 0.4221 & 0.4783 & 20.29 & 20.26 \\
\midrule
\sacson & DINO-Reg, 25 epochs & 0.4173 & 0.4568 & 0.4195 & 0.4679 & 124.55 & 149.24 \\
 & DINO-Reg, 47 epochs & 0.3886 & 0.4294 & 0.3842 & 0.4288 & 100.55 & 122.86 \\
 & DINO-Reg, 50 epochs & 0.3865 & 0.4275 & 0.3817 & 0.4266 & 98.76 & 120.85 \\
 & \paper \M{1}, $S{=}50$ & 0.3433 & 0.3786 & 0.3618 & 0.3916 & 19.12 & 20.96 \\
\midrule
\scand & DINO-Reg, 25 epochs & 0.5289 & 0.5640 & 0.4846 & 0.5196 & 134.97 & 144.72 \\
 & DINO-Reg, 47 epochs & 0.4884 & 0.5191 & 0.4783 & 0.5100 & 98.44 & 103.41 \\
 & DINO-Reg, 50 epochs & 0.4847 & 0.5146 & 0.4785 & 0.5100 & 95.23 & 99.81 \\
 & \paper \M{1}, $S{=}50$ & 0.3991 & 0.4587 & 0.4564 & 0.5151 & 31.12 & 35.65 \\
\midrule
Mean & DINO-Reg, 25 epochs & 0.4820 & 0.5341 & 0.4617 & 0.5153 & 142.35 & 170.57 \\
 & DINO-Reg, 47 epochs & 0.4480 & 0.5017 & 0.4369 & 0.4869 & 105.90 & 126.92 \\
 & DINO-Reg, 50 epochs & 0.4452 & 0.4988 & 0.4355 & 0.4854 & 103.16 & 123.46 \\
 & \paper \M{1}, $S{=}50$ & 0.3757 & 0.4325 & 0.4134 & 0.4617 & 23.51 & 25.62 \\


==> tab/gen/supp_t2_reg_plan_body.tex <==
DINO-Reg, 25 epochs & $1.753\pm0.018$ & $2.965\pm0.058$ & $1.229\pm0.026$ & $0.449\pm0.005$ & $0.731\pm0.007$ & $0.318\pm0.005$ \\
DINO-Reg, 47 epochs & $2.198\pm0.026$ & $3.080\pm0.022$ & $1.230\pm0.026$ & $0.538\pm0.005$ & $0.750\pm0.003$ & $0.318\pm0.006$ \\
DINO-Reg, 50 epochs (Table~2) & $2.234\pm0.005$ & $3.090\pm0.033$ & $1.223\pm0.024$ & $0.544\pm0.002$ & $0.755\pm0.004$ & $0.318\pm0.005$ \\
\addlinespace[2pt]
\paper \M{1}, $S{=}2$ (1 NFE) & $1.249\pm0.010$ & $2.811\pm0.027$ & $0.996\pm0.012$ & $0.376\pm0.003$ & $0.705\pm0.005$ & $0.284\pm0.002$ \\
\paper \M{1}, $S{=}5$ (4 NFEs) & $1.266\pm0.016$ & $2.749\pm0.077$ & $1.011\pm0.014$ & $0.363\pm0.001$ & $0.692\pm0.015$ & $0.283\pm0.001$ \\
\mono, $S{=}50$ (49 NFEs) & $1.363\pm0.010$ & $2.838\pm0.024$ & $1.038\pm0.023$ & $0.367\pm0.001$ & $0.698\pm0.003$ & $0.288\pm0.002$ \\


==> tab/gen/supp_t2_reg_plan_ci_body.tex <==
\multicolumn{4}{@{}l}{\emph{\ate}} \\
DINO-Reg (50) $-$ \M{1}@2 (1 NFE) & $+0.985$\sig [$+0.895$, $+1.072$] & $+0.280$\sig [$+0.186$, $+0.374$] & $+0.227$\sig [$+0.192$, $+0.265$] \\
DINO-Reg (50) $-$ \M{1}@5 (4 NFEs) & $+0.967$\sig [$+0.887$, $+1.050$] & $+0.342$\sig [$+0.259$, $+0.432$] & $+0.213$\sig [$+0.178$, $+0.248$] \\
DINO-Reg (50) $-$ {\mono}@50 (49 NFEs) & $+0.871$\sig [$+0.796$, $+0.948$] & $+0.253$\sig [$+0.165$, $+0.342$] & $+0.185$\sig [$+0.148$, $+0.219$] \\
DINO-Reg (50) $-$ DINO-Reg (47) & $+0.036$\sig [$+0.018$, $+0.054$] & $+0.011$ [$-0.019$, $+0.041$] & $-0.007$ [$-0.018$, $+0.006$] \\
DINO-Reg (50) $-$ DINO-Reg (25) & $+0.480$\sig [$+0.414$, $+0.545$] & $+0.126$\sig [$+0.060$, $+0.192$] & $-0.006$ [$-0.038$, $+0.026$] \\
DINO-Reg (47) $-$ DINO-Reg (25) & $+0.445$\sig [$+0.379$, $+0.506$] & $+0.115$\sig [$+0.053$, $+0.180$] & $+0.000$ [$-0.031$, $+0.031$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{\rpe}} \\
DINO-Reg (50) $-$ \M{1}@2 (1 NFE) & $+0.168$\sig [$+0.154$, $+0.183$] & $+0.050$\sig [$+0.034$, $+0.064$] & $+0.034$\sig [$+0.028$, $+0.041$] \\
DINO-Reg (50) $-$ \M{1}@5 (4 NFEs) & $+0.181$\sig [$+0.166$, $+0.196$] & $+0.063$\sig [$+0.048$, $+0.079$] & $+0.035$\sig [$+0.029$, $+0.040$] \\
DINO-Reg (50) $-$ {\mono}@50 (49 NFEs) & $+0.177$\sig [$+0.164$, $+0.192$] & $+0.057$\sig [$+0.041$, $+0.073$] & $+0.030$\sig [$+0.025$, $+0.036$] \\
DINO-Reg (50) $-$ DINO-Reg (47) & $+0.006$\sig [$+0.003$, $+0.010$] & $+0.005$ [$-0.001$, $+0.011$] & $-0.000$ [$-0.002$, $+0.002$] \\
DINO-Reg (50) $-$ DINO-Reg (25) & $+0.095$\sig [$+0.084$, $+0.107$] & $+0.024$\sig [$+0.011$, $+0.037$] & $-0.000$ [$-0.005$, $+0.005$] \\
DINO-Reg (47) $-$ DINO-Reg (25) & $+0.089$\sig [$+0.078$, $+0.100$] & $+0.019$\sig [$+0.007$, $+0.032$] & $+0.000$ [$-0.005$, $+0.005$] \\


==> tab/gen/supp_t2_reg_tok_body.tex <==
\multicolumn{16}{@{}l}{\emph{1\,s: one-shot prediction vs.\ frame 3 of the rollout (four chained 0.25\,s steps, 1.00\,s)}} \\
DINO-Reg, 25 epochs & 0.167 & 0.184 & $+0.017$ & 0.380 & 0.416 & 0.137 & 0.150 & $+0.013$ & 0.321 & 0.350 & 0.241 & 0.271 & $+0.030$ & 0.542 & 0.610 \\
DINO-Reg, 47 epochs & 0.167 & 0.184 & $+0.017$ & 0.380 & 0.417 & 0.133 & 0.148 & $+0.015$ & 0.313 & 0.346 & 0.266 & 0.292 & $+0.026$ & 0.603 & 0.665 \\
DINO-Reg, 50 epochs & 0.167 & 0.184 & $+0.016$ & 0.381 & 0.417 & 0.133 & 0.148 & $+0.015$ & 0.313 & 0.346 & 0.269 & 0.294 & $+0.026$ & 0.610 & 0.671 \\
\addlinespace[2pt]
\M{1}, $S{=}2$ (1) & 0.170 & 0.181 & $+0.011$ & 0.385 & 0.408 & 0.145 & 0.156 & $+0.011$ & 0.338 & 0.361 & 0.191 & 0.206 & $+0.015$ & 0.436 & 0.471 \\
\M{1}, $S{=}3$ (2) & 0.198 & 0.207 & $+0.009$ & 0.453 & 0.474 & 0.164 & 0.174 & $+0.010$ & 0.386 & 0.408 & 0.216 & 0.227 & $+0.011$ & 0.499 & 0.526 \\
\M{1}, $S{=}5$ (4) & 0.228 & 0.235 & $+0.008$ & 0.534 & 0.554 & 0.188 & 0.196 & $+0.008$ & 0.449 & 0.469 & 0.243 & 0.249 & $+0.006$ & 0.575 & 0.592 \\
\M{1}, $S{=}50$ (49) & 0.272 & 0.282 & $+0.010$ & 0.667 & 0.692 & 0.229 & 0.237 & $+0.008$ & 0.569 & 0.589 & 0.286 & 0.287 & $+0.001$ & 0.711 & 0.715 \\
\midrule
\multicolumn{16}{@{}l}{\emph{2\,s: one-shot prediction vs.\ frame 8 of the rollout (nine chained 0.25\,s steps, 2.25\,s)}} \\
DINO-Reg, 25 epochs & 0.174 & 0.226 & $+0.052$ & 0.394 & 0.504 & 0.137 & 0.174 & $+0.037$ & 0.320 & 0.401 & 0.249 & 0.305 & $+0.056$ & 0.559 & 0.685 \\
DINO-Reg, 47 epochs & 0.175 & 0.228 & $+0.053$ & 0.397 & 0.513 & 0.133 & 0.178 & $+0.045$ & 0.312 & 0.413 & 0.271 & 0.322 & $+0.051$ & 0.614 & 0.736 \\
DINO-Reg, 50 epochs & 0.175 & 0.228 & $+0.053$ & 0.398 & 0.514 & 0.133 & 0.178 & $+0.045$ & 0.313 & 0.414 & 0.274 & 0.324 & $+0.050$ & 0.621 & 0.741 \\
\addlinespace[2pt]
\M{1}, $S{=}2$ (1) & 0.178 & 0.212 & $+0.035$ & 0.402 & 0.476 & 0.146 & 0.176 & $+0.030$ & 0.342 & 0.406 & 0.208 & 0.249 & $+0.040$ & 0.472 & 0.564 \\
\M{1}, $S{=}3$ (2) & 0.207 & 0.239 & $+0.032$ & 0.474 & 0.548 & 0.166 & 0.191 & $+0.026$ & 0.390 & 0.449 & 0.236 & 0.270 & $+0.034$ & 0.541 & 0.623 \\
\M{1}, $S{=}5$ (4) & 0.238 & 0.267 & $+0.029$ & 0.558 & 0.629 & 0.190 & 0.213 & $+0.023$ & 0.454 & 0.509 & 0.265 & 0.291 & $+0.026$ & 0.624 & 0.691 \\
\M{1}, $S{=}50$ (49) & 0.282 & 0.314 & $+0.031$ & 0.691 & 0.770 & 0.233 & 0.252 & $+0.019$ & 0.577 & 0.626 & 0.310 & 0.328 & $+0.019$ & 0.768 & 0.819 \\


==> tab/gen/supp_t2_reg_turns_body.tex <==
\recon & Q1 straightest (0.07--1.14) & 0.89 & 1.087 & 1.075 & 1.048 & 1.053 & 1.232 & 1.205 & 1.210 & $+0.134$\sig \ci{$+0.061$, $+0.203$} & $+0.162$\sig \ci{$+0.077$, $+0.248$} & $+0.157$\sig \ci{$+0.082$, $+0.236$} \\
 & Q2 (1.15--2.20) & 1.25 & 1.161 & 1.132 & 1.139 & 1.116 & 1.419 & 1.629 & 1.671 & $+0.539$\sig \ci{$+0.427$, $+0.654$} & $+0.532$\sig \ci{$+0.419$, $+0.648$} & $+0.555$\sig \ci{$+0.445$, $+0.672$} \\
 & Q3 (2.20--3.53) & 1.73 & 1.314 & 1.155 & 1.172 & 1.140 & 1.577 & 2.321 & 2.369 & $+1.214$\sig \ci{$+1.084$, $+1.330$} & $+1.197$\sig \ci{$+1.062$, $+1.321$} & $+1.229$\sig \ci{$+1.102$, $+1.355$} \\
 & Q4 sharpest (3.54--8.95) & 2.68 & 1.889 & 1.703 & 1.639 & 1.653 & 2.786 & 3.638 & 3.686 & $+1.983$\sig \ci{$+1.835$, $+2.118$} & $+2.048$\sig \ci{$+1.882$, $+2.195$} & $+2.033$\sig \ci{$+1.861$, $+2.190$} \\
\midrule
\sacson & Q1 straightest (0.00--0.60) & 2.67 & 1.747 & 1.644 & 1.688 & 1.469 & 1.875 & 1.953 & 1.959 & $+0.315$\sig \ci{$+0.169$, $+0.458$} & $+0.271$\sig \ci{$+0.125$, $+0.416$} & $+0.490$\sig \ci{$+0.344$, $+0.633$} \\
 & Q2 (0.61--1.49) & 3.60 & 2.693 & 2.690 & 2.701 & 2.538 & 2.881 & 2.878 & 2.921 & $+0.232$\sig \ci{$+0.054$, $+0.392$} & $+0.220$\sig \ci{$+0.068$, $+0.382$} & $+0.383$\sig \ci{$+0.218$, $+0.557$} \\
 & Q3 (1.51--3.28) & 3.92 & 3.028 & 2.890 & 2.924 & 2.758 & 3.092 & 3.371 & 3.346 & $+0.456$\sig \ci{$+0.278$, $+0.637$} & $+0.422$\sig \ci{$+0.226$, $+0.637$} & $+0.588$\sig \ci{$+0.411$, $+0.768$} \\
 & Q4 sharpest (3.29--11.86) & 4.93 & 3.883 & 3.771 & 3.931 & 3.743 & 4.010 & 4.118 & 4.136 & $+0.365$\sig \ci{$+0.160$, $+0.553$} & $+0.205$\sig \ci{$+0.006$, $+0.426$} & $+0.393$\sig \ci{$+0.178$, $+0.607$} \\
\midrule
\scand & Q1 straightest (0.01--0.07) & 0.55 & 0.782 & 0.791 & 0.814 & 0.781 & 1.077 & 1.048 & 1.045 & $+0.254$\sig \ci{$+0.182$, $+0.316$} & $+0.231$\sig \ci{$+0.166$, $+0.298$} & $+0.264$\sig \ci{$+0.205$, $+0.322$} \\
 & Q2 (0.07--0.18) & 0.75 & 1.010 & 0.943 & 0.917 & 0.957 & 1.179 & 1.185 & 1.172 & $+0.229$\sig \ci{$+0.168$, $+0.295$} & $+0.255$\sig \ci{$+0.180$, $+0.330$} & $+0.214$\sig \ci{$+0.140$, $+0.292$} \\
 & Q3 (0.18--0.54) & 0.75 & 0.976 & 0.972 & 0.951 & 0.967 & 1.109 & 1.124 & 1.128 & $+0.156$\sig \ci{$+0.086$, $+0.223$} & $+0.177$\sig \ci{$+0.107$, $+0.252$} & $+0.161$\sig \ci{$+0.085$, $+0.237$} \\
 & Q4 sharpest (0.54--5.11) & 1.29 & 1.381 & 1.335 & 1.304 & 1.309 & 1.552 & 1.562 & 1.548 & $+0.212$\sig \ci{$+0.122$, $+0.295$} & $+0.243$\sig \ci{$+0.148$, $+0.327$} & $+0.239$\sig \ci{$+0.143$, $+0.324$} \\


==> tab/gen/supp_t2_seed1_ci_body.tex <==
\multicolumn{4}{@{}l}{\emph{(a) Granularity at a fixed step count, training seed 1}} \\
\M{1}@50 $-$ {\mono}@50 & $-0.001$ [$-0.028$, $+0.028$] & $-0.065$\sig [$-0.133$, $-0.000$] & $-0.023$ [$-0.052$, $+0.003$] \\
\M{1}@5 $-$ {\mono}@5 & $-0.018$ [$-0.042$, $+0.008$] & $-0.038$ [$-0.101$, $+0.023$] & $-0.033$\sig [$-0.059$, $-0.007$] \\
\M{1}@3 $-$ {\mono}@3 & $-0.019$ [$-0.042$, $+0.008$] & $+0.002$ [$-0.069$, $+0.074$] & $-0.075$\sig [$-0.104$, $-0.048$] \\
\M{1}@2 $-$ {\mono}@2 & $+0.008$ [$-0.022$, $+0.037$] & $-0.042$ [$-0.128$, $+0.047$] & $-0.091$\sig [$-0.126$, $-0.058$] \\
\M{1}@3 (2 draws) $-$ {\mono}@3 (2 draws) & $-0.015$ [$-0.039$, $+0.009$] & $-0.017$ [$-0.085$, $+0.053$] & $-0.060$\sig [$-0.090$, $-0.032$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{(b) Granularity at a fixed step count, training seed 0 (primary runs; as in \cref{tab:s-pooled})}} \\
\M{1}@50 $-$ {\mono}@50 & $+0.005$ [$-0.021$, $+0.032$] & $-0.002$ [$-0.064$, $+0.053$] & $-0.012$ [$-0.036$, $+0.013$] \\
\M{1}@5 $-$ {\mono}@5 & $-0.029$\sig [$-0.054$, $-0.004$] & $-0.008$ [$-0.065$, $+0.052$] & $-0.021$ [$-0.044$, $+0.003$] \\
\M{1}@3 $-$ {\mono}@3 & $-0.024$ [$-0.049$, $+0.001$] & $+0.053$ [$-0.009$, $+0.113$] & $-0.060$\sig [$-0.090$, $-0.033$] \\
\M{1}@2 $-$ {\mono}@2 & $-0.015$ [$-0.044$, $+0.016$] & $+0.102$\sig [$+0.032$, $+0.175$] & $-0.098$\sig [$-0.128$, $-0.069$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{(c) Step reduction, training seed 1}} \\
\M{1}@5 $-$ \M{1}@50 & $-0.087$\sig [$-0.116$, $-0.061$] & $-0.100$\sig [$-0.149$, $-0.053$] & $-0.001$ [$-0.024$, $+0.019$] \\
\M{1}@3 $-$ \M{1}@50 & $-0.132$\sig [$-0.168$, $-0.099$] & $-0.090$\sig [$-0.150$, $-0.030$] & $-0.022$ [$-0.050$, $+0.003$] \\
\M{1}@2 $-$ \M{1}@50 & $-0.115$\sig [$-0.154$, $-0.081$] & $-0.099$\sig [$-0.179$, $-0.020$] & $-0.030$\sig [$-0.057$, $-0.002$] \\
{\mono}@5 $-$ {\mono}@50 & $-0.069$\sig [$-0.095$, $-0.046$] & $-0.128$\sig [$-0.175$, $-0.075$] & $+0.009$ [$-0.014$, $+0.032$] \\
{\mono}@3 $-$ {\mono}@50 & $-0.114$\sig [$-0.145$, $-0.084$] & $-0.157$\sig [$-0.217$, $-0.098$] & $+0.029$\sig [$+0.003$, $+0.057$] \\
{\mono}@2 $-$ {\mono}@50 & $-0.123$\sig [$-0.163$, $-0.088$] & $-0.122$\sig [$-0.197$, $-0.051$] & $+0.038$\sig [$+0.007$, $+0.071$] \\
{\mono}@3 (2 draws) $-$ {\mono}@50 & $-0.122$\sig [$-0.152$, $-0.093$] & $-0.232$\sig [$-0.295$, $-0.169$] & $+0.023$ [$-0.003$, $+0.050$] \\
\M{1}@5 $-$ {\mono}@50 & $-0.087$\sig [$-0.116$, $-0.058$] & $-0.165$\sig [$-0.227$, $-0.100$] & $-0.025$ [$-0.055$, $+0.005$] \\
\M{1}@2 $-$ {\mono}@50 & $-0.115$\sig [$-0.153$, $-0.083$] & $-0.164$\sig [$-0.261$, $-0.069$] & $-0.054$\sig [$-0.085$, $-0.022$] \\
\M{1}@3 (2 draws) $-$ {\mono}@50 & $-0.138$\sig [$-0.171$, $-0.105$] & $-0.249$\sig [$-0.322$, $-0.174$] & $-0.037$\sig [$-0.066$, $-0.008$] \\
\M{1}@3 (2 draws) $-$ \M{1}@3 & $-0.005$ [$-0.020$, $+0.010$] & $-0.094$\sig [$-0.135$, $-0.050$] & $+0.009$ [$-0.009$, $+0.029$] \\
{\mono}@3 (2 draws) $-$ {\mono}@3 & $-0.008$ [$-0.023$, $+0.008$] & $-0.075$\sig [$-0.112$, $-0.039$] & $-0.006$ [$-0.022$, $+0.011$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{(d) Training seed 1 minus training seed 0, same model and $S$}} \\
\M{1}@50 & $+0.009$ [$-0.015$, $+0.037$] & $+0.008$ [$-0.044$, $+0.063$] & $-0.014$ [$-0.037$, $+0.010$] \\
\M{1}@5 & $+0.024$\sig [$+0.001$, $+0.049$] & $-0.005$ [$-0.066$, $+0.053$] & $+0.000$ [$-0.026$, $+0.025$] \\
\M{1}@3 & $-0.002$ [$-0.024$, $+0.024$] & $+0.039$ [$-0.024$, $+0.104$] & $-0.008$ [$-0.031$, $+0.016$] \\
\M{1}@2 & $+0.013$ [$-0.013$, $+0.041$] & $-0.066$ [$-0.136$, $+0.004$] & $-0.015$ [$-0.041$, $+0.014$] \\
\M{1}@3 (2 draws) & $-0.000$ [$-0.024$, $+0.023$] & $+0.033$ [$-0.028$, $+0.096$] & $-0.005$ [$-0.031$, $+0.024$] \\
{\mono}@50 & $+0.015$ [$-0.013$, $+0.040$] & $+0.071$\sig [$+0.015$, $+0.130$] & $-0.002$ [$-0.028$, $+0.024$] \\
{\mono}@5 & $+0.013$ [$-0.009$, $+0.033$] & $+0.024$ [$-0.029$, $+0.084$] & $+0.013$ [$-0.012$, $+0.036$] \\
{\mono}@3 & $-0.007$ [$-0.031$, $+0.017$] & $+0.090$\sig [$+0.023$, $+0.152$] & $+0.006$ [$-0.020$, $+0.033$] \\
{\mono}@2 & $-0.010$ [$-0.038$, $+0.019$] & $+0.078$\sig [$+0.004$, $+0.149$] & $-0.021$ [$-0.050$, $+0.009$] \\
\midrule
\multicolumn{4}{@{}l}{\emph{(e) Difference of contrasts between training seeds (seed 1 minus seed 0)}} \\
(\M{1}@2 $-$ {\mono}@50) & $-0.002$ [$-0.037$, $+0.035$] & $-0.137$\sig [$-0.235$, $-0.048$] & $-0.012$ [$-0.049$, $+0.027$] \\
(\M{1}@5 $-$ {\mono}@50) & $+0.009$ [$-0.025$, $+0.043$] & $-0.076$ [$-0.157$, $+0.002$] & $+0.003$ [$-0.034$, $+0.038$] \\
(\M{1}@5 $-$ \M{1}@50) & $+0.015$ [$-0.017$, $+0.047$] & $-0.013$ [$-0.078$, $+0.047$] & $+0.014$ [$-0.016$, $+0.043$] \\
({\mono}@5 $-$ {\mono}@50) & $-0.002$ [$-0.033$, $+0.029$] & $-0.047$ [$-0.112$, $+0.014$] & $+0.015$ [$-0.016$, $+0.046$] \\


==> tab/gen/supp_t2_seed1_gen_body.tex <==
\recon & \mono & 50 (49) & 0.3736 & 0.4523 & 0.4133 & 0.4716 & 18.86 & 18.42 & 0.3734 & 0.4518 & 0.4127 & 0.4714 & 18.62 & 18.59 \\
 & \paper \M{4} & 50 (49) & 0.3794 & 0.4569 & 0.4184 & 0.4761 & 19.09 & 19.07 & 0.3804 & 0.4574 & 0.4187 & 0.4762 & 19.53 & 19.10 \\
 & \paper \M{1} & 50 (49) & 0.3846 & 0.4602 & 0.4221 & 0.4783 & 20.29 & 20.26 & 0.3855 & 0.4620 & 0.4216 & 0.4782 & 20.94 & 20.87 \\
 & \mono & 5 (4) & 0.3694 & 0.4531 & 0.3919 & 0.4535 & 21.69 & 21.81 & 0.3678 & 0.4519 & 0.3912 & 0.4536 & 21.96 & 21.57 \\
 & \paper \M{4} & 5 (4) & 0.3753 & 0.4582 & 0.3966 & 0.4575 & 22.91 & 22.85 & 0.3759 & 0.4582 & 0.3967 & 0.4573 & 23.13 & 22.88 \\
 & \paper \M{1} & 5 (4) & 0.3819 & 0.4627 & 0.4010 & 0.4604 & 25.00 & 24.98 & 0.3825 & 0.4641 & 0.4007 & 0.4604 & 25.35 & 25.55 \\
\midrule
\sacson & \mono & 50 (49) & 0.3232 & 0.3605 & 0.3452 & 0.3775 & 16.51 & 17.82 & 0.3230 & 0.3601 & 0.3445 & 0.3775 & 16.69 & 17.47 \\
 & \paper \M{4} & 50 (49) & 0.3331 & 0.3692 & 0.3535 & 0.3853 & 17.08 & 18.69 & 0.3324 & 0.3696 & 0.3534 & 0.3853 & 17.27 & 18.75 \\
 & \paper \M{1} & 50 (49) & 0.3433 & 0.3786 & 0.3618 & 0.3916 & 19.12 & 20.96 & 0.3423 & 0.3786 & 0.3607 & 0.3910 & 18.78 & 20.63 \\
 & \mono & 5 (4) & 0.3103 & 0.3470 & 0.3258 & 0.3580 & 20.49 & 22.45 & 0.3108 & 0.3471 & 0.3257 & 0.3582 & 20.68 & 22.14 \\
 & \paper \M{4} & 5 (4) & 0.3202 & 0.3555 & 0.3348 & 0.3661 & 21.64 & 23.67 & 0.3200 & 0.3553 & 0.3347 & 0.3656 & 21.88 & 23.89 \\
 & \paper \M{1} & 5 (4) & 0.3313 & 0.3654 & 0.3438 & 0.3739 & 24.70 & 26.61 & 0.3302 & 0.3643 & 0.3430 & 0.3727 & 24.40 & 26.87 \\
\midrule
\scand & \mono & 50 (49) & 0.4053 & 0.4565 & 0.4583 & 0.5087 & 28.55 & 31.28 & 0.4080 & 0.4579 & 0.4601 & 0.5107 & 29.29 & 32.02 \\
 & \paper \M{4} & 50 (49) & 0.3991 & 0.4580 & 0.4548 & 0.5122 & 29.05 & 32.78 & 0.4010 & 0.4579 & 0.4560 & 0.5114 & 29.53 & 33.55 \\
 & \paper \M{1} & 50 (49) & 0.3991 & 0.4587 & 0.4564 & 0.5151 & 31.12 & 35.65 & 0.4014 & 0.4594 & 0.4568 & 0.5134 & 31.53 & 35.94 \\
 & \mono & 5 (4) & 0.3975 & 0.4500 & 0.4438 & 0.4959 & 33.26 & 35.46 & 0.3998 & 0.4519 & 0.4453 & 0.4977 & 34.02 & 36.66 \\
 & \paper \M{4} & 5 (4) & 0.3887 & 0.4501 & 0.4378 & 0.4974 & 34.10 & 37.32 & 0.3905 & 0.4503 & 0.4390 & 0.4972 & 34.36 & 38.07 \\
 & \paper \M{1} & 5 (4) & 0.3894 & 0.4517 & 0.4399 & 0.5010 & 36.42 & 41.35 & 0.3913 & 0.4521 & 0.4402 & 0.4997 & 36.89 & 41.83 \\
\midrule
Three-dataset mean & \mono & 50 (49) & 0.3674 & 0.4231 & 0.4056 & 0.4526 & 21.30 & 22.51 & 0.3681 & 0.4233 & 0.4058 & 0.4532 & 21.54 & 22.70 \\
 & \paper \M{4} & 50 (49) & 0.3705 & 0.4280 & 0.4089 & 0.4579 & 21.74 & 23.51 & 0.3713 & 0.4283 & 0.4094 & 0.4577 & 22.11 & 23.80 \\
 & \paper \M{1} & 50 (49) & 0.3757 & 0.4325 & 0.4134 & 0.4617 & 23.51 & 25.62 & 0.3764 & 0.4333 & 0.4131 & 0.4609 & 23.75 & 25.81 \\
 & \mono & 5 (4) & 0.3590 & 0.4167 & 0.3872 & 0.4358 & 25.15 & 26.57 & 0.3595 & 0.4170 & 0.3874 & 0.4365 & 25.56 & 26.79 \\
 & \paper \M{4} & 5 (4) & 0.3614 & 0.4213 & 0.3897 & 0.4403 & 26.22 & 27.95 & 0.3622 & 0.4213 & 0.3901 & 0.4400 & 26.46 & 28.28 \\
 & \paper \M{1} & 5 (4) & 0.3675 & 0.4266 & 0.3949 & 0.4451 & 28.71 & 30.98 & 0.3680 & 0.4268 & 0.3946 & 0.4442 & 28.88 & 31.42 \\


==> tab/gen/supp_t2_seed1_plan_body.tex <==
\multicolumn{8}{@{}l}{\emph{Training seed 1}} \\
\mono & 50 (49) & $1.378\pm0.019$ & $2.909\pm0.017$ & $1.035\pm0.017$ & $0.370\pm0.004$ & $0.714\pm0.002$ & $0.288\pm0.002$ \\
 & 5 (4) & $1.308\pm0.025$ & $2.781\pm0.015$ & $1.044\pm0.021$ & $0.366\pm0.003$ & $0.700\pm0.003$ & $0.290\pm0.001$ \\
 & 3 (2) & $1.264\pm0.006$ & $2.752\pm0.023$ & $1.064\pm0.005$ & $0.363\pm0.002$ & $0.698\pm0.003$ & $0.293\pm0.001$ \\
 & 2 (1) & $1.255\pm0.005$ & $2.787\pm0.066$ & $1.073\pm0.017$ & $0.366\pm0.003$ & $0.702\pm0.010$ & $0.294\pm0.004$ \\
 & $2{\times}3$ ($2{\times}2$) & $1.255\pm0.012$ & $2.677\pm0.010$ & $1.059\pm0.003$ & -- & -- & -- \\
\paper \M{1} & 50 (49) & $1.377\pm0.035$ & $2.843\pm0.021$ & $1.012\pm0.016$ & $0.367\pm0.007$ & $0.697\pm0.006$ & $0.283\pm0.003$ \\
 & 5 (4) & $1.290\pm0.011$ & $2.743\pm0.001$ & $1.011\pm0.022$ & $0.365\pm0.001$ & $0.691\pm0.007$ & $0.283\pm0.001$ \\
 & 3 (2) & $1.245\pm0.004$ & $2.754\pm0.040$ & $0.990\pm0.038$ & $0.367\pm0.001$ & $0.692\pm0.006$ & $0.281\pm0.005$ \\
 & 2 (1) & $1.262\pm0.005$ & $2.745\pm0.017$ & $0.982\pm0.029$ & $0.375\pm0.001$ & $0.690\pm0.008$ & $0.281\pm0.002$ \\
 & $2{\times}3$ ($2{\times}2$) & $1.240\pm0.014$ & $2.660\pm0.029$ & $0.999\pm0.012$ & -- & -- & -- \\
\midrule
\multicolumn{8}{@{}l}{\emph{Training seed 0 (primary runs, for reference)}} \\
\mono & 50 (49) & $1.363\pm0.010$ & $2.838\pm0.024$ & $1.038\pm0.023$ & $0.367\pm0.001$ & $0.698\pm0.003$ & $0.288\pm0.002$ \\
 & 5 (4) & $1.295\pm0.013$ & $2.756\pm0.034$ & $1.032\pm0.023$ & $0.363\pm0.003$ & $0.690\pm0.003$ & $0.287\pm0.002$ \\
 & 3 (2) & $1.271\pm0.017$ & $2.662\pm0.059$ & $1.058\pm0.015$ & $0.366\pm0.003$ & $0.683\pm0.007$ & $0.292\pm0.002$ \\
 & 2 (1) & $1.265\pm0.003$ & $2.708\pm0.039$ & $1.094\pm0.015$ & $0.371\pm0.003$ & $0.685\pm0.001$ & $0.297\pm0.002$ \\
\paper \M{1} & 50 (49) & $1.368\pm0.024$ & $2.836\pm0.059$ & $1.026\pm0.015$ & $0.367\pm0.003$ & $0.694\pm0.010$ & $0.285\pm0.002$ \\
 & 5 (4) & $1.266\pm0.016$ & $2.749\pm0.077$ & $1.011\pm0.014$ & $0.363\pm0.001$ & $0.692\pm0.015$ & $0.283\pm0.001$ \\
 & 3 (2) & $1.247\pm0.004$ & $2.715\pm0.036$ & $0.997\pm0.022$ & $0.370\pm0.001$ & $0.688\pm0.005$ & $0.282\pm0.002$ \\
 & 2 (1) & $1.249\pm0.010$ & $2.811\pm0.027$ & $0.996\pm0.012$ & $0.376\pm0.003$ & $0.705\pm0.005$ & $0.284\pm0.002$ \\
 & $2{\times}3$ ($2{\times}2$) & $1.240\pm0.005$ & $2.627\pm0.031$ & $1.003\pm0.032$ & -- & -- & -- \\


==> tab/gen/supp_turns_body.tex <==
\recon & Q1 straightest (0.07--1.14) & 0.89 & 0.81 & 1.09 & 1.08 & 1.08 & 1.08 & 1.06 & 1.05 & 1.05 & $0.00$ \ci{$-0.04$, $+0.04$} & $-0.02$ \ci{$-0.06$, $+0.03$} & $-0.03$ \ci{$-0.07$, $+0.03$} & $-0.03$ \ci{$-0.09$, $+0.03$} & $+0.01$ \ci{$-0.04$, $+0.04$} & $-0.01$ \ci{$-0.04$, $+0.03$} \\
 & Q2 (1.15--2.20) & 1.25 & 1.17 & 1.16 & 1.10 & 1.17 & 1.13 & 1.11 & 1.12 & 1.14 & $-0.03$ \ci{$-0.08$, $+0.02$} & $-0.05$\sig \ci{$-0.10$, $-0.00$} & $+0.01$ \ci{$-0.04$, $+0.05$} & $-0.03$ \ci{$-0.08$, $+0.03$} & $-0.02$ \ci{$-0.06$, $+0.01$} & $-0.06$\sig \ci{$-0.10$, $-0.01$} \\
 & Q3 (2.20--3.53) & 1.73 & 1.69 & 1.31 & 1.24 & 1.28 & 1.16 & 1.15 & 1.14 & 1.17 & $-0.12$\sig \ci{$-0.16$, $-0.07$} & $-0.13$\sig \ci{$-0.18$, $-0.08$} & $+0.02$ \ci{$-0.03$, $+0.06$} & $-0.10$\sig \ci{$-0.16$, $-0.04$} & $-0.03$ \ci{$-0.07$, $+0.01$} & $-0.08$\sig \ci{$-0.13$, $-0.03$} \\
 & Q4 sharpest (3.54--8.95) & 2.68 & 2.68 & 1.89 & 1.76 & 1.95 & 1.70 & 1.67 & 1.65 & 1.64 & $-0.25$\sig \ci{$-0.31$, $-0.19$} & $-0.28$\sig \ci{$-0.35$, $-0.21$} & $-0.06$ \ci{$-0.14$, $+0.01$} & $-0.31$\sig \ci{$-0.40$, $-0.22$} & $+0.01$ \ci{$-0.04$, $+0.07$} & $-0.13$\sig \ci{$-0.18$, $-0.07$} \\
\midrule
\sacson & Q1 straightest (0.00--0.60) & 2.67 & 1.19 & 1.75 & 1.65 & 1.72 & 1.64 & 1.54 & 1.47 & 1.69 & $-0.07$ \ci{$-0.15$, $+0.01$} & $-0.18$\sig \ci{$-0.28$, $-0.09$} & $+0.04$ \ci{$-0.08$, $+0.16$} & $-0.03$ \ci{$-0.17$, $+0.12$} & $-0.22$\sig \ci{$-0.35$, $-0.12$} & $-0.09$\sig \ci{$-0.17$, $-0.02$} \\
 & Q2 (0.61--1.49) & 3.60 & 1.65 & 2.69 & 2.66 & 2.76 & 2.69 & 2.64 & 2.54 & 2.70 & $-0.07$ \ci{$-0.16$, $+0.04$} & $-0.12$ \ci{$-0.23$, $+0.00$} & $+0.01$ \ci{$-0.12$, $+0.14$} & $-0.05$ \ci{$-0.21$, $+0.09$} & $-0.16$\sig \ci{$-0.27$, $-0.05$} & $-0.04$ \ci{$-0.12$, $+0.06$} \\
 & Q3 (1.51--3.28) & 3.92 & 2.31 & 3.03 & 2.93 & 3.00 & 2.89 & 2.88 & 2.76 & 2.92 & $-0.11$\sig \ci{$-0.21$, $-0.01$} & $-0.12$ \ci{$-0.24$, $+0.00$} & $+0.03$ \ci{$-0.11$, $+0.17$} & $-0.07$ \ci{$-0.22$, $+0.08$} & $-0.17$\sig \ci{$-0.28$, $-0.05$} & $-0.10$\sig \ci{$-0.20$, $-0.00$} \\
 & Q4 sharpest (3.29--11.86) & 4.93 & 3.82 & 3.88 & 3.79 & 3.87 & 3.77 & 3.80 & 3.74 & 3.93 & $-0.10$ \ci{$-0.19$, $+0.00$} & $-0.07$ \ci{$-0.21$, $+0.06$} & $+0.16$\sig \ci{$+0.01$, $+0.32$} & $+0.06$ \ci{$-0.11$, $+0.24$} & $-0.19$\sig \ci{$-0.32$, $-0.06$} & $-0.09$ \ci{$-0.19$, $+0.01$} \\
\midrule
\scand & Q1 straightest (0.01--0.07) & 0.55 & 0.55 & 0.78 & 0.79 & 0.78 & 0.79 & 0.80 & 0.78 & 0.81 & $+0.01$ \ci{$-0.03$, $+0.05$} & $+0.01$ \ci{$-0.04$, $+0.06$} & $+0.02$ \ci{$-0.03$, $+0.07$} & $+0.03$ \ci{$-0.02$, $+0.08$} & $-0.03$ \ci{$-0.07$, $+0.01$} & $0.00$ \ci{$-0.04$, $+0.04$} \\
 & Q2 (0.07--0.18) & 0.75 & 0.75 & 1.01 & 1.00 & 0.97 & 0.94 & 0.93 & 0.96 & 0.92 & $-0.03$ \ci{$-0.08$, $+0.01$} & $-0.04$ \ci{$-0.09$, $+0.01$} & $-0.03$ \ci{$-0.08$, $+0.02$} & $-0.06$ \ci{$-0.12$, $+0.00$} & $+0.04$ \ci{$-0.01$, $+0.09$} & $-0.01$ \ci{$-0.05$, $+0.03$} \\
 & Q3 (0.18--0.54) & 0.75 & 0.75 & 0.98 & 0.97 & 1.01 & 0.97 & 0.95 & 0.97 & 0.95 & $-0.04$ \ci{$-0.08$, $+0.01$} & $-0.06$\sig \ci{$-0.11$, $-0.01$} & $-0.02$ \ci{$-0.08$, $+0.03$} & $-0.06$\sig \ci{$-0.12$, $-0.00$} & $+0.02$ \ci{$-0.03$, $+0.06$} & $-0.01$ \ci{$-0.05$, $+0.04$} \\
 & Q4 sharpest (0.54--5.11) & 1.29 & 1.29 & 1.38 & 1.37 & 1.33 & 1.34 & 1.31 & 1.31 & 1.30 & $0.00$ \ci{$-0.05$, $+0.05$} & $-0.02$ \ci{$-0.07$, $+0.03$} & $-0.03$ \ci{$-0.08$, $+0.02$} & $-0.03$ \ci{$-0.09$, $+0.03$} & $0.00$ \ci{$-0.04$, $+0.05$} & $-0.02$ \ci{$-0.06$, $+0.03$} \\


==> tab/gen/tab4_full_body.tex <==
Euler, $S{=}50$ (49 NFEs) & 47{,}040 & 1.37 & 2.78 & 1.01 & 1.38 & 2.81 & 1.02 & 1.35 & 2.85 & 1.01 \\
Euler, $S{=}50$, CRN (49 NFEs) & 47{,}040 & 1.32 & 2.85 & 1.02 & -- & -- & -- & 1.33 & 2.79 & 1.05 \\
Euler, $S{=}10$ (9 NFEs) & 8{,}640 & 1.32 & 2.74 & 0.99 & 1.31 & 2.76 & 1.00 & 1.32 & 2.80 & 1.00 \\
Euler, $S{=}10$, CRN (9 NFEs) & 8{,}640 & 1.26\sig & 2.78 & 0.99 & -- & -- & -- & 1.32 & 2.70 & 1.04 \\
Euler, $S{=}5$ (4 NFEs) & 3{,}840 & 1.26 & 2.68 & 1.00 & 1.27 & 2.71 & 1.00 & 1.29 & 2.78 & 1.01 \\
Euler, $S{=}5$, CRN (4 NFEs) & 3{,}840 & 1.26 & 2.75 & 1.02 & 1.25 & 2.72 & 1.00 & 1.29 & 2.65\sig & 1.04 \\
Euler, $S{=}5$, $\bm{\epsilon}{=}\bm{0}$ (4 NFEs) & 3{,}840 & 1.48\sig & 3.19\sig & 1.03 & -- & -- & -- & -- & -- & -- \\
Euler, $S{=}5$, fused SDPA (4 NFEs) & 3{,}840 & -- & 2.69 & -- & -- & -- & -- & -- & 2.78 & -- \\
Uniform Euler ($\alpha{=}1$, 4 NFEs) & 3{,}840 & 1.27 & 2.70 & 0.99 & -- & -- & -- & 1.30 & 2.75 & 1.01 \\
Uniform Heun ($\alpha{=}1$, 4 NFEs) & 3{,}840 & 1.33\sig & 2.75 & 1.01 & -- & -- & -- & 1.34\sig & 2.73 & 1.01 \\
Uniform midpoint ($\alpha{=}1$, 4 NFEs) & 3{,}840 & 1.36\sig & 2.75 & 1.01 & -- & -- & -- & 1.37\sig & 2.79 & 1.04 \\
Euler, $S{=}3$ (2 NFEs) & 1{,}920 & 1.24 & 2.67 & 1.01 & 1.25 & 2.69 & 1.01 & 1.27 & 2.73 & 1.07 \\
Heun, $S{=}3$ (4 NFEs) & 3{,}840 & 1.41\sig & 2.80\sig & 0.99 & -- & -- & -- & 1.38\sig & 2.83 & 1.05\sig \\
Midpoint, $S{=}3$ (4 NFEs) & 3{,}840 & 1.37\sig & 2.78\sig & 1.01 & -- & -- & -- & 1.39\sig & 2.78 & 1.03 \\
Euler, $S{=}2$ (1 NFE) & 960 & 1.26 & 2.80\sig & 0.99 & 1.25 & 2.76 & 0.99 & 1.26 & 2.71 & 1.10\sig \\
Euler, $S{=}2$, CRN (1 NFE) & 960 & 1.25 & 2.80 & 1.00 & -- & -- & -- & 1.25 & 2.70 & 1.08 \\
Euler, $S{=}2$, $\bm{\epsilon}{=}\bm{0}$ (1 NFE) & 960 & 1.40\sig & 3.11\sig & 1.10\sig & -- & -- & -- & -- & -- & -- \\


==> tab/gen/tab4_full_ci_body.tex <==
Euler, $S{=}50$ (49 NFEs) & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Euler, $S{=}50$, CRN (49 NFEs) & $-0.05$ [$-0.10$, $+0.00$] & $+0.07$ [$-0.03$, $+0.18$] & $+0.01$ [$-0.04$, $+0.05$] & -- & -- & -- & $-0.02$ [$-0.07$, $+0.03$] & $-0.06$ [$-0.16$, $+0.05$] & $+0.04$ [$-0.01$, $+0.08$] \\
Euler, $S{=}10$ (9 NFEs) & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Euler, $S{=}10$, CRN (9 NFEs) & $-0.06$ [$-0.11$, $-0.02$] & $+0.04$ [$-0.05$, $+0.13$] & $0.00$ [$-0.04$, $+0.04$] & -- & -- & -- & $0.00$ [$-0.05$, $+0.04$] & $-0.10$ [$-0.20$, $+0.01$] & $+0.04$ [$-0.00$, $+0.09$] \\
Euler, $S{=}5$ (4 NFEs) & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Euler, $S{=}5$, CRN (4 NFEs) & $+0.01$ [$-0.03$, $+0.05$] & $+0.07$ [$-0.02$, $+0.16$] & $+0.02$ [$-0.02$, $+0.06$] & $-0.02$ [$-0.06$, $+0.02$] & $+0.01$ [$-0.07$, $+0.10$] & $+0.01$ [$-0.03$, $+0.05$] & $-0.01$ [$-0.05$, $+0.03$] & $-0.12$ [$-0.22$, $-0.02$] & $+0.04$ [$-0.00$, $+0.08$] \\
Euler, $S{=}5$, $\bm{\epsilon}{=}\bm{0}$ (4 NFEs) & $+0.22$ [$+0.16$, $+0.28$] & $+0.52$ [$+0.39$, $+0.65$] & $+0.03$ [$-0.02$, $+0.07$] & -- & -- & -- & -- & -- & -- \\
Euler, $S{=}5$, fused SDPA (4 NFEs) & -- & $+0.01$ [$-0.00$, $+0.03$] & -- & -- & -- & -- & -- & $0.00$ [$-0.01$, $+0.01$] & -- \\
Uniform Euler ($\alpha{=}1$, 4 NFEs) & $+0.02$ [$-0.02$, $+0.06$] & $+0.03$ [$-0.06$, $+0.12$] & $-0.01$ [$-0.05$, $+0.03$] & -- & -- & -- & $+0.01$ [$-0.03$, $+0.04$] & $-0.03$ [$-0.11$, $+0.06$] & $0.00$ [$-0.04$, $+0.04$] \\
Uniform Heun ($\alpha{=}1$, 4 NFEs) & $+0.07$ [$+0.03$, $+0.12$] & $+0.07$ [$-0.02$, $+0.16$] & $+0.01$ [$-0.03$, $+0.05$] & -- & -- & -- & $+0.05$ [$+0.01$, $+0.09$] & $-0.04$ [$-0.13$, $+0.05$] & $0.00$ [$-0.04$, $+0.04$] \\
Uniform midpoint ($\alpha{=}1$, 4 NFEs) & $+0.10$ [$+0.06$, $+0.14$] & $+0.07$ [$-0.00$, $+0.15$] & $+0.01$ [$-0.03$, $+0.06$] & -- & -- & -- & $+0.07$ [$+0.03$, $+0.11$] & $+0.02$ [$-0.06$, $+0.11$] & $+0.03$ [$-0.00$, $+0.07$] \\
Euler, $S{=}3$ (2 NFEs) & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Heun, $S{=}3$ (4 NFEs) & $+0.15$ [$+0.10$, $+0.20$] & $+0.12$ [$+0.04$, $+0.20$] & $-0.01$ [$-0.05$, $+0.03$] & -- & -- & -- & $+0.09$ [$+0.05$, $+0.13$] & $+0.05$ [$-0.03$, $+0.14$] & $+0.04$ [$+0.00$, $+0.07$] \\
Midpoint, $S{=}3$ (4 NFEs) & $+0.11$ [$+0.07$, $+0.15$] & $+0.10$ [$+0.03$, $+0.18$] & $+0.01$ [$-0.02$, $+0.05$] & -- & -- & -- & $+0.09$ [$+0.05$, $+0.13$] & $0.00$ [$-0.07$, $+0.07$] & $+0.02$ [$-0.01$, $+0.06$] \\
Euler, $S{=}2$ (1 NFE) & $0.00$ [$-0.04$, $+0.04$] & $+0.13$ [$+0.03$, $+0.23$] & $-0.01$ [$-0.06$, $+0.03$] & $-0.02$ [$-0.06$, $+0.02$] & $+0.05$ [$-0.05$, $+0.15$] & $0.00$ [$-0.05$, $+0.04$] & $-0.03$ [$-0.08$, $+0.01$] & $-0.07$ [$-0.16$, $+0.03$] & $+0.09$ [$+0.05$, $+0.14$] \\
Euler, $S{=}2$, CRN (1 NFE) & $-0.01$ [$-0.03$, $+0.02$] & $-0.01$ [$-0.08$, $+0.06$] & $+0.01$ [$-0.01$, $+0.03$] & -- & -- & -- & $-0.01$ [$-0.03$, $+0.01$] & $-0.01$ [$-0.07$, $+0.05$] & $-0.02$ [$-0.05$, $+0.01$] \\
Euler, $S{=}2$, $\bm{\epsilon}{=}\bm{0}$ (1 NFE) & $+0.14$ [$+0.09$, $+0.18$] & $+0.30$ [$+0.17$, $+0.44$] & $+0.11$ [$+0.06$, $+0.16$] & -- & -- & -- & -- & -- & -- \\


==> tab/gen/turns_main_body.tex <==
\recon & straightest ($\le$1.14) & 0.89 & 1.09 & 1.08 & 1.08 & 1.08 & 1.05 & 1.05 & $0.00$ & $-0.03$ & $+0.01$ \\
 & sharpest ($\ge$3.54) & 2.68 & 1.89 & 1.76 & 1.95 & 1.70 & 1.65 & 1.64 & $-0.25$\tsig & $-0.06$ & $+0.01$ \\
\midrule
\sacson & straightest ($\le$0.60) & 2.67 & 1.75 & 1.65 & 1.72 & 1.64 & 1.47 & 1.69 & $-0.07$ & $+0.04$ & $-0.22$\tsig \\
 & sharpest ($\ge$3.29) & 4.93 & 3.88 & 3.79 & 3.87 & 3.77 & 3.74 & 3.93 & $-0.10$ & $+0.16$\tsig & $-0.19$\tsig \\
\midrule
\sacson-cal. & straightest ($\le$0.60) & 1.19 & 1.56 & 1.54 & 1.71 & 1.52 & 1.48 & 1.70 & -- & -- & -- \\
 & sharpest ($\ge$3.29) & 3.82 & 3.19 & 3.11 & 3.22 & 3.13 & 3.07 & 3.23 & $-0.09$ & $+0.10$ & $-0.16$\tsig \\

